Gating is Weighting: Understanding Gated Linear Attention through In-context Learning

Linear attention methods offer a compelling alternative to softmax attention due to their efficiency in recurrent decoding. Recent research has focused on enhancing standard linear attention by incorporating gating while retaining its computational benefits. Such Gated Linear Attention (GLA) architectures include competitive models such as Mamba and RWKV. In this work, we investigate the in-context learning capabilities of the GLA model and make the following contributions. We show that a multilayer GLA can implement a general class of Weighted Preconditioned Gradient Descent (WPGD) algorithms with data-dependent weights. These weights are induced by the gating mechanism and the input, enabling the model to control the contribution of individual tokens to prediction. To further understand the mechanics of this weighting, we introduce a novel data model with multitask prompts and characterize the optimization landscape of learning a WPGD algorithm. Under mild conditions, we establish the existence and uniqueness (up to scaling) of a global minimum, corresponding to a unique WPGD solution. Finally, we translate these findings to explore the optimization landscape of GLA and shed light on how gating facilitates context-aware learning and when it is provably better than vanilla linear attention.

==> colm_sec/gla_landscape.tex <==
\section{Optimization landscape of GLA}\label{gla sec}
%
% In Section~\ref{sec plain wpgd}, we demonstrated that GLA implements a data-dependent WPGD algorithm. Building on this, in Section~\ref{sec:optim gd}, we analyze the optimization landscape for minimizing the one-step WPGD risk (cf.~\eqref{eqn:wpgd:risk}) and show that a unique solution (up to rescaling) achieves the global minimum of the WPGD algorithm. However, in GLA, the search space for $\bom$ is restricted and data-dependent, meaning that $\Lc_\wpgd^\st$ in \eqref{eqn:wpgd:risk} represents the best possible risk a GLA model can achieve. 
In this section, we analyze the loss landscape for training a one-layer GLA model and explore the scenarios under which GLA can reach the optimal WPGD risk.
%
%
\subsection{Multi-task prompt model}\label{sec:multi p}
Following Definitions~\ref{corr task def} and \ref{def:multitask}, we consider the multi-task prompt setting with \( K \) correlated tasks \((\bt_k)_{k=1}^K\) and one query task \(\bt\).
% with distribution $\Nc(0,\Iden)$. 
For each correlated task $k\in[K]$, a prompt of length \( n_k \) is drawn, consisting of IID input-label pairs  \(\{(\x_{ik}, y_{ik})\}_{i=1}^{n_k}\) where $y_{ik}\sim\Nc(\bt_k^\top\x_{ik},\sigma^2)$ 
to obtain sequence $\Z_k=\begin{bmatrix}
    \x_{1k}&\cdots&\x_{n_k,k}\\y_{1k}&\cdots&y_{n_k,k}
\end{bmatrix}^\top$. Let \( n := \sum_{k=1}^K n_k \). 
% The query is given by \(\z_{n+1} = [\x_{n+1}~~0]^\top\) with the corresponding label \( y_{n+1} \sim \Nc(\x_{n+1}^\top\bt, \sigma^2) \). All the features $\x_{ik}$ for $i\in[n_k],k\in[K]$ and query feature $\x_{n+1}$ are IID sampled from $\Nc(\zerobb,\bSi)$.

These sequences \((\Z_k)_{k=1}^K\), along with the query token \(\z_{n+1}= [\x_{n+1}~~0]^\top\), are concatenated to form a single prompt \(\Z\). Recall \eqref{eq:GLA}, and let \( f_{\gla}(\Z) \) denote the GLA prediction as defined in Theorem~\ref{thm:gla=wpgd}. Additionally, consider the model construction in \eqref{att mtx res}, where \(\Pq, \Pk \in \R^{d \times d}\) are trainable parameters. The GLA optimization problem is described as follows:
\begin{equation}\label{eqn:gla:risk}
\begin{split}
&\Lc_\gla^\st := \min_{\Pk, \Pq\in\R^{d\times d}, G\in\Gc}~\Lc_\gla(\Pk, \Pq, G), \quad \\
&\text{where} \quad \Lc_\gla(\Pk, \Pq, G) = \E\left[\left(y - f_{\gla}(\Z)\right)^2\right]. 
\end{split}
\end{equation}
Here, $G(\cdot)$ represents the gating function and $\Gc$ denotes the function search space, which is determined by the chosen gating strategies (cf. Table 1 in \cite{yang2023gated}). %\da{is the gating function a vector. Should it be $\mathbf{g}$. Is $\Gc$ defined previously? }


Note that 1) the task vectors $(\bt_k)_{k=1}^K$ are not explicitly shown in the prompt,
% but are latent  within the random samples $(\x_i^{(k)}, y_i^{(k)})$, 
2) in-context features $\x_{ik}$ are randomly drawn, and 3) the gating function is applied to the tokens $(\Z_k)_{k=1}^K$. Given the above three evidences, the implicit weighting induced by the GLA model varies across different prompts, and it prevents the GLA from learning the optimal weighting. 
To address this, we introduce delimiters to mark the boundary of each task. 
Let $(\db_k)_{k=1}^{K}$ be the delimiters that determine stop of the tasks.
% We will assume that there are delimiters that separate the task sequences. 
Specifically, the final prompt is given by 
\begin{align}
\Z=\begin{bmatrix}\Z_1^\top&\db_1&\cdots&\Z_K^\top&\db_K&\z_{n+1}\end{bmatrix}^\top.\label{mtl prompt}
\end{align}
Additionally, to decouple the influence of gating and data, we envision that each token is $\z_i=[\x_i^\top~~y_i~~\cb_i^\top]^\top$ where $\cb_i\neq\zerobb\in\R^p$ is the contextual features with $p$ being its dimension and $(\x_i,y_i)$ are the data features. 
Let $\cbb_0,\cdots,\cbb_K\in\R^p$ be $K+1$ contextual feature vectors.
\begin{itemize}
    \item For task prompts $\Z_k$: Contextual features are set to a fixed vector $\cbb_0\neq \zerobb$.
    \item For delimiters $\db_k$: Data features (e.g., $\x_i,y_i$) are set to zero  so that $\db_k=[\zerobb_{d+1}^\top~\cbb_k^\top]^\top$.
    % where $\cbb_k\in\R^p$ denotes the \yl{contextual feature}\asrnote{Is it clear what we mean by `context vector'?}.
\end{itemize}
Explicit delimiters have been utilized in addressing real-world problems \citep{wang2024one,asai2022attempt,dun2023sweeping} due to their ability to improve efficiency and enhance generalization, particularly in task-mixture or multi-document scenarios. To further motivate the introduction of \((\db_k)_{k=1}^K\), we present in Figure~\ref{fig:k=2} the results of GLA training with and without delimiters, represented by the red and green curves, respectively. The black dashed curves indicate the optimal WPGD loss, \(\Lc^\st_\wpgd\), under different scenarios. Notably, training GLA without delimiters (the green solid curve) performs strictly worse. In contrast, training with delimiters can achieve optimal performance under certain conditions (see Figures~\ref{fig:0 1}, \ref{fig:0.2 0.8}, and \ref{fig:0.5 0.5}). Theorem~\ref{thm:gla optim}, presented in the next section, provides a theoretical explanation for these observations, including the misalignment observed in Figure~\ref{fig:0.8 0.2}. 
% Further discussion and experimental details are provided in Section~\ref{sec:gla optim} and Appendix~\ref{sec:exp}.








\input{sec/fig_k=2}

\subsection{Loss landscape of one-layer GLA}\label{sec:gla optim}
Given the input tokens with extended dimension, to ensure that GLA still implements WPGD as in Theorem~\ref{thm:gla=wpgd}, we propose the following model construction. 
\begin{align}\Wt_k=\begin{bmatrix}
    \Wk&\zerobb\\
    \zerobb&\zerobb
\end{bmatrix},\quad\Wt_q=\begin{bmatrix}
    \Wq&\zerobb\\\zerobb&\zerobb
\end{bmatrix},\quad\text{and}\quad\tilde\W_v=\begin{bmatrix}\Wv&\zerobb\\\zerobb&\zerobb\end{bmatrix}.\label{att mtx res delimiter}
\end{align}
Here, $\Wt_{k,q,v}\in\R^{(d+p+1)\times(d+p+1)}$ and $\W_{k,q,v}\in\R^{(d+1)\times(d+1)}$ are constructed via \eqref{att mtx res}. 
The main idea is to set the last $p$ rows and columns of attention matrices to zeros, ensuring that the delimiters do not affect the final prediction. 
\begin{assumption}\label{assum delimiter gate}
Contextual feature vectors $\cbb_0,\cdots,\cbb_K$ are linearly independent, and 
% \end{assumption}
% \begin{assumption}\label{assum gate}
    activation function $\phi(z):\R\to[0,1]$ is continuous, satisfying $\phi(-\infty) = 0$ and $\phi(+\infty) = 1$.
\end{assumption}
\begin{assumption}\label{assum order}
    The correlation between context tasks $(\bt_k)_{k=1}^K$ and query task $\bt$ satisfies $\E[\bt_i^\top\bt_j]=0$ and $\E[\bt_i^\top\bt]\leq\E[\bt_j^\top\bt]$ for  all $1\leq i\leq j\leq K$.
\end{assumption}
% \yl{The activation function $\phi(\cdot)$ in Assumption~\ref{assum delimiter gate} introduces nonlinearity to the gating function (see Theorem~\ref{thm:gla optim}).}
Given context examples $\{(\X_k,\y_k):=(\x_{ik},y_{ik})_{i=1}^{n_k}\}_{k=1}^{K}$, define the concatenated data $(\X,\y)$:
\begin{align}
\X=\begin{bmatrix}
    \X_1^\top&\cdots&\X_K^\top
\end{bmatrix}^\top\in\R^{n\times d}, \quad\text{and}\quad\y=\begin{bmatrix}
    \y_1^\top&\cdots&\y_K^\top
\end{bmatrix}^\top\in\R^{n}.\label{K task X y}
\end{align}
Based on the assumptions above, we are able to establish the equivalence between optimizing one-layer GLA and optimizing one-step WPGD predictor {under scalar gating}.
\begin{theorem} [{Scalar Gating}]\label{thm:gla optim}
Suppose Assumption~\ref{assum delimiter gate} holds. Recap the function $\Lc_\wpgd(\Pb,\bom)$ from \eqref{eqn:wpgd:risk} with dataset $(\X,\y)$ defined in \eqref{K task X y}. Consider \eqref{eq:GLA} with input prompt $\Z$ defined in \eqref{mtl prompt}, the model constructions described in \eqref{att mtx res delimiter}, and  scalar gating $G(\z)=\phi(\w_g^\top\z)\onebb_{(d+p+1)\times(d+p+1)}$, where $\w_g$ is a trainable parameter. Then, the optimal risk $\Lc^\st_\gla$ defined in \eqref{eqn:gla:risk} obeys
    \begin{align}
{\Lc_\gla^\st=\Lc_{\wpgd}^{\st,\Wc}, \quad\text{where}\quad\Lc_{\wpgd}^{\st,\Wc}:=\min_{\Pb\in\R^{d\times d},\bom\in\Wc}~\Lc_\wpgd(\Pb,\bom).}\label{gla=wpgd W}
    \end{align}
    Here, 
    $
    \Wc:=\left\{\left[\omega_1\onebb_{n_1}^\top~\cdots~\omega_K\onebb_{n_K}^\top\right]^\top\in\R^{n}~\Big|~0\leq\omega_i\leq\omega_j\leq1,~\forall 1\leq i\leq j\leq K\right\}.
    $
    
    Additionally, suppose Assumption~\ref{assum order} holds and $n_i=n_j$, for all  $i,j\in[K]$. Let $\Lc_\wpgd^\st$ be the optimal WPGD risk (cf.~\eqref{eqn:wpgd:risk}). Then  $\Lc^\st_\gla$ satisfies
    \begin{align}
    \Lc_\gla^\st=\Lc_\wpgd^\st.\label{gla=wpgd}
    \end{align}
\end{theorem}
% Recall the gating function $g(\z):=g(\w_g^\top\z)$ from \eqref{eqn:gla:risk}. 
Assumption~\ref{assum delimiter gate} ensures that any $\bom$ in $\Wc$ can be achieved by an appropriate choice of gating parameters. Furthermore, Assumption~\ref{assum order} guarantees that the optimal choice of $\bom$ under the WPGD objective lies within the search space $\Wc$. The proof is provided in Appendix~\ref{app:proof gla optim}.

In Figure~\ref{fig:k=2}, we conduct model training to validate our findings. Consider the setting where $K=2$ and let $(r_1, r_2) = \left(\E[\bt_1^\top\bt]/d, \E[\bt_2^\top\bt]/d\right)$. In Figures~\ref{fig:0 1}, \ref{fig:0.2 0.8}, and \ref{fig:0.5 0.5}, Assumption~\ref{assum order} holds, and the GLA results (shown in solid red) align with the optimal WPGD risk (represented by the dashed black), validating \eqref{gla=wpgd}. However, in Figure~\ref{fig:0.8 0.2}, since $r_1 > r_2$, Assumption~\ref{assum order} does not hold, and as a result, the optimal GLA loss $\Lc^\st_\gla$ obtained from \eqref{gla=wpgd W} is lower than the optimal WPGD loss $\Lc^\st_\wpgd$. Further details are deferred to Appendix~\ref{sec:exp}.

\paragraph*{Loss landscape of vector gating.} Till now,  our discussion has focused on the scalar gating setting.
% , where the gating is assumed to take the form $g(\z)\onebb\onebb^\top$ for a scalar $g(\z)$.
It is important to highlight that, even in the scalar-weighting context, analyzing the WPGD problem remains non-trivial due to the joint optimization over $(\Pb, \bom)$. However, as demonstrated in Theorem~\ref{thm:gla optim}, scalar gating can only express weightings within the set $\Wc$. If Assumption~\ref{assum order} does not hold, $\Lc^\st_\gla$ cannot achieve the optimal WPGD loss (see the misalignment between red solid curve, presenting $\Lc^\st_\gla$, and black dashed curve, presenting $\Lc^\st_\wpgd$ in Figure~\ref{fig:0.8 0.2}). We argue that vector gating overcomes this limitation by applying distinct weighting mechanisms across different dimensions, facilitating stronger expressivity. 
% \YL{Mention linear prediction head}
\begin{theorem} [{Vector Gating}] \label{thm:gla optim vector}
 Suppose Assumption~\ref{assum delimiter gate} holds.  
 Consider \eqref{eq:GLA} with input prompt $\Z$ from \eqref{mtl prompt}, the model constructions from \eqref{att mtx res delimiter} but with $\tilde\W_v=[\zerobb_{(d+p+1)\times d}~~\ub~~\zerobb_{(d+p+1)\times p}]^\top$, and a vector gating $G(\z)=\phi(\W_g\z)\onebb^\top_{d+p+1}$. Recap Problem \eqref{eqn:gla:risk} with prediction defined as  $f_{\gla}(\Z):=\ob_{n+1}^\top\hb$, where $\hb\in\R^{d+p+1}$ is a linear prediction head. Here, $\ub$, $\W_g$ and $\hb$ are trainable parameters. Let $\Lc_{\gla\text{-}v}^\st$ denote its optimal risk, and $\Lc_{\wpgd}^\st$ be defined as in \eqref{eqn:wpgd:risk}.
    % Consider a linear head $\hb$ such that prediction is given via $f_{\gla}(\Z)=\ob_{n+1}^\top\hb$. Let gating defined as $\Gb_i=g(\z_i)\onebb^\top$ with $g(\z_i)\in\R^{d+p+1}$. 
    % Then, the optimal risk obeys
    Then, $
    \Lc_{\gla\text{-}v}^\st=\Lc_\wpgd^\st$.
\end{theorem}
{In Theorem~\ref{thm:gla optim}, the equivalence between $\Lc_{\gla}^\st$ and $\Lc_{\wpgd}^\st$ is established only when both Assumptions~\ref{assum delimiter gate} and \ref{assum order} are satisfied. In contrast, Theorem~\ref{thm:gla optim vector} demonstrates that applying vector gating requires only Assumption~\ref{assum delimiter gate} to establish $\Lc_{\gla\text{-}v}^\st = \Lc_{\wpgd}^\st$. Specifically, under the bounded activation model of Assumption~\ref{assum delimiter gate}, scalar gating is unable to express non-monotonic weighting schemes. For instance, suppose there are two tasks: Even if Task 1 is more relevant to the query, Assumption~\ref{assum delimiter gate} will assign a higher (or equal) weight to examples in Task 2 resulting in sub-optimal prediction. Theorem \ref{thm:gla optim vector} shows that vector gating can avoid such bottlenecks by potentially encoding tasks in distinct subspaces. 
To verify these intuitions}, in Figure~\ref{fig:0.8 0.2}, we train a GLA model with vector gating 
% where gating is given via $\Gb_i=g(\z_i)\onebb^\top$ and $g(\z_i)=\W_g\z_i\in\R^{d+p+1}$. The vector gating
and results are presented in cyan curve, which outperform the scalar gating results (red solid) and align with the optimal WPGD loss (black dashed). %The proof of Theorem \ref{thm:gla optim vector} is provided in Appendix~\ref{app:gla optim vector}.




\begin{comment}

\textbf{Gating function.} For simplicity, let us consider a sigmoid gating model which can pass or supress the state via $\Gb_i=g_i\onebb_{d\times d}$ where $g_i=\sigma(\w_{gate}^\top\z_i) \in (0,1)$. Our intuition is as follows:
\begin{itemize}
\item Suppose tasks are entirely uncorrelated, that is, $\bt_i$ does not inform $\bt_{j}$ for $j\neq i$. Then, we expect that when the model encounters $\db_k$, the gating mechanism will suppress the history by setting $g(\db_k)=0$ however when encountered by actual task tokens, the model will pass the history by setting $g(\x_i)=1$ and start accumulating the state to infer the task vector in-context.
\begin{itemize}
    \item Under this model, we expect that, the gating weights will converge to a max-margin separator that separates the task tokens from the delimiters to enforce $g(\db_k)=0$ and $g(\x_i)=1$.
\end{itemize}
\item When tasks are correlated, the model can selectively pass the history. In that case, depending on the correlation level between $\bt_1,\bt_2$, the model will intuitively learn a fixed forgetting level $g(\db_1)=\alpha$ so that features of $\bt_1$ can help estimate $\bt_2$ to an extent.
\end{itemize}

Finally, we assume gating only applies on the context. This ensures that the weighting $\bom$ is independent of the features $\X,\y$ and easier to analyze. Gathering these, we have the following claim. Let
\[ 
\X=[\X_1^\top~\dots~\X_K^\top]^\top,\quad \y=[\y_1^\top~\dots~\y_K^\top]^\top
\]
We claim that attention learns WPGD with weights $\bom$ as in \eqref{wpgd}. Here, the crucial aspect is form of the weighting. $\bom$ takes the following clean form \SO{exponents might be off by 1}.
\[ 
\bom_{kL+i}=g(\dbb_0^\top \w_{gate})^{kL+i-1}\prod_{j=1}^{k-1} g(\dbb_i^\top \w_{gate})
\]
This form follows from the fact that, until $kL+i$, the model observes $kL+i-1$ standard datapoints and $k-1$ delimiters. Now using the shorthand notation $g_0=g(\cb^\top \w_{gate})$ and $g_i=g(\dbb_i^\top \w_{gate})$, we can rewrite
\begin{align}
\bom_{kL+i}=g_0^{kL+i-1} \prod_{j=1}^{k-1}g_i.\label{bom orig}
\end{align}
Whenever $(\dbb_i)_{i=0}^{L-1}$ are linearly independent and gating function is sufficiently expressive\footnote{In case of sigmoid, it can express everything in the [0,1] interval but not the whole real line.}, gating function can be treated as \textbf{unconstrained variables}, that is, model can express any scalars $\g=(g_i)_{i=0}^{K-1}$ of its choice. As a result, the analysis of GLA directly relates to the \emph{risk of optimally-weighted PGD}. 

\noindent\textbf{Change of variable trick.} To further simplify \eqref{bom orig} let us apply a change of variable relying $g'_k\gets g_0^L g_k$ and $\tilde{g}_k=\prod_{j=1}^{k-1}g'_j$. Through this, we obtain the simplified form
\begin{align}
\bom_{kL+i}=g_0^{i-1} \prod_{j=1}^{k-1}g'_j=g_0^{i-1} \tilde{g}_k.\label{bom CoR}
\end{align}
This simplified forms highlight the fact that, along the data sequence $\Z_i$, gating results in an exponential filter whereas and delimeters act as a multiplicative adjustments that can be summarized as $g'_k$ or the aggregate multiplier $\tilde{g}_k$. When $\g=(g_k)_{k=1}^K$ are unconstrained variables, \eqref{bom CoR} is precisely equivalent to the original form \eqref{bom orig}.
 

Suppose $(\X_i,\y_i)_{i=1}^{K}$ are all datasets with IID samples and consider the objective 
\begin{align}\tag{GatingLoss}
\Lc(\Pb,\g)=\sum_{k=1}^K \Lc_k(\Pb,\g):=\sum_{k=1}^K\E[(y^{(k)}_L-\li\x^{(k)}_L,\Pb\Xb_k(\bom^{(k)}\odot\yb_k)\ri)^2.\label{GWPGD}
\end{align}
Above $\Lc_k$ is the $k$'th loss induced by the $i$'th sequences prediction, $\Xb_k,\yb_k$ are the concatenations of $(\X_j,y_j)_{j=1}^k$ (but not including the token $\z^{(k)}_L$) and $\bom^{(k)}$ is the first $Lk-1$ entries of the weight vector $\bom$.

With the formulation of \eqref{GWPGD}, the problem (essentially) boils down to the landscape analysis of the population risk of WPGD to obtain the optimal gating weights $\g=(g_i)_{i=0}^{K-1}$. A major starting/exposition point for the analysis is directly studying the simplified change-of-variable form \eqref{bom CoR} under the unconstrained variable assumption. This brings us to the following claim when the task vectors $(\bt_k)_{k=1}^K$ are independent.

\begin{claim} The optimal choice of $\g$ is given by $g_0=1$ and $g_{k\geq 1}=0$.
\end{claim}
Note that, if this claim holds for the unconstrained variable setting, it automatically holds for the sigmoid gating because optimal function for unconstrained is also optimal for the [0,1] constrained sigmoidal.

Once this is proven, I believe we can then deduce the GLA-WPGD equivance by utilizing the facts that (i) $g_i$'s are independent of features (in fact, even deterministic) and (ii) odd moment statistics that appear in linear attention will vanish. Note that, if task vectors are dependent, then most likely the following claim holds.

\begin{claim}\label{claim2} The optimal choice of $\g$ is given by $g_0=1$ and $g_{k\geq 1}=\alpha_k$ for a suitable choice.
\end{claim}
I recommend proving the above claim first in the setting of $K=2$.

Finally, as a variation of \eqref{GWPGD}, rather than adding $K$ loss terms, we can directly focus on analyzing the $K$'th loss. That is, rather than \eqref{GWPGD}, we study
\begin{align}\tag{SingleLoss}
\Lc(\Pb,\g)=\E[(y^{(K)}_L-\li\x^{(K)}_L,\Pb\Xb_K(\bom^{(K)}\odot\yb_K)\ri)^2.\label{SWPGD}
\end{align}



\subsection{Relaxing Assumptions on Gating (requires fleshing out)}

Above we have been using the assumption that gating only depends on $\cb_t$ and not on $\x_t$. This might appear too simplistic because it kind of circumvents the data-dependent nature of gating by using context $\cb_t$ rather than features $\x_t$. I believe this can be avoided. The basic idea is the following claim:
\begin{claim} Suppose $\y=\X\bt_\star$ and $\omega_t=g(\w_{wgt}^\top\x_t)$. Suppose $\x,\bt\sim\Nn(0,\Iden_d)$. Consider the estimator $\hat\bt=\Pb\X^\top(\bom\odot\y)$. Choosing $g(\cdot)=\texttt{constant}$ is a near-optimal weighting strategy to minimize risk. That is, you want to weight all samples equally and data-dependent weighting don't buy anything (except perhaps $\order{1/d}$ improvements).
\end{claim}
\noindent\textbf{Proof idea.} The proof should follow from rotational invariance of gaussian. Specifically, gating can only contribute to the estimation of $\bt$ along the subspace $\w_{wgt}$. Over the remaining $d-1$ dimensional subspace, unless all weights are equal, gating will only reduce the performance because $\omega_t$ is independent of $\x^\perp_t$, which is the projection of $\x_t$ on the orthogonal complement of $\w_{wgt}$. Note that analysis of gating is more tricky because $\omega_t$ is multiplication of all earlier $g(\w_{gate}^\top\x_{\tau<t})$ rather than a direct function of $\x_t$. \SO{In fact, the actual gated prediction seems nonlinear in the query $\x$. Based on \eqref{eq:GLA}, the prediction seems to include gating of $\x$, namely, $\hat y=g(\x)\x^\top \hat\bt$. This has to be written very accurately.}

\noindent\textbf{Suggestion.} Even if we don't want to worry about proving/formalizing this aspect, we can run experiments to verify the claim. We simply need to run experiment where gating is allowed to be function of $\x_t$ and demonstrate that result doesn't change.

%$\x_t\perp \cb_t$ to keep things clean. I think this assumption is not needed. We only need $\x_t$ of data to be separable from $\db_i$'s

%Finally, imagine the contexts of the individual data points are also arbitrary and resulting gate-weightings are unconstrained. In that case, we can view $\bom$ as a fully unconstrained vector in $\R^{KL}$ and gating becomes precisely equal to weighted.
%and formalize Claim \ref{claim2} for $K=2$.
%\noindent\textbf{Critical assumption 1:} Gating is only a function of $\cb_i$ whereas attention weights only apply on $[\x_i,y_i]$. This can be guaranteed by assuming $\x_i,\cb_i$ lie on orthogonal subspaces. That is, tokens effectively have the form $\z_i=[y_i,\x_i,\cb_i]$.


%\begin{itemize}
%\end{itemize}

\end{comment}

==> colm_sec/gla_to_gd.tex <==
%Connecting Gated Linear Attention to Gradient Methods
\section{What gradient methods can GLA emulate?}\label{sec plain wpgd}
In this section, we investigate the ICL capabilities of {{GLA}} and show that under suitable 
%model construction 
{instantiations of model weights}, GLA can implement \textit{data-dependent} WPGD. 

\subsection{{GLA as a data-dependent WPGD predictor}}  

\paragraph*{Data-Dependent WPGD.}  
Given $\X$ and $\y$ as defined in \eqref{PGD loss}, consider the weighted least squares objective $\Lc(\bt)=\sum_{i=1}^n \omega_i\cdot (y_i-\bt^\top \x_i)^2$ with weights $\bom=[\omega_1,\omega_2,~\cdots,~\omega_n]^\top\in\R^n$. To optimize this, we use gradient descent (GD) starting from zero initialization, $\bt_0 = \zerobb$ with a step size of $\eta = 1/2$. One step of standard GD is given by
\begin{align*}%\label{eqn:gd}
    \bt_1 = \bt_0 - \eta\nabla\Lc(\bt_0)=\sum_{i=1}^n \omega_i \cdot \x_i y_i=\X^\top (\bom\odot\y).
\end{align*}  
Given a test/query feature $\x$, the corresponding prediction is $\hat{y} = \x^\top \hat{\bt}$ where $ \hat{\bt} = \bt_1$. Additionally, if we were using PGD with a {preconditioning matrix $\Pb\in\R^{d\times d}$, $\bt_0 = \zerobb$, and $\eta = 1/2$, then a single iteration results in}
\begin{equation}\label{eqn:gd:wpgd-basic}
\hat{y} = \x^\top \hat{\bt}, \quad \text{where} \quad {\hat{\bt}  =\bt_0 -  \eta \Pb \nabla\Lc(\bt_0)}= \Pb \X^\top (\bom\odot\y).
\end{equation}
Above is the basic {\emph{sample-wise} WPGD} predictor which weights individual datapoints, in contrast to the PGD predictor as presented in \eqref{PGD pred}. It turns out, \emph{vector-valued gating} can facilitate a more general estimator which weights individual coordinates. To this aim,  we introduce an extension 
% of \eqref{eqn:gd:pred}
as follows: Let $\Pb_1, \Pb_2 \in \R^{d \times d}$ denote the preconditioning matrices, and let $\bOm \in \R^{n \times d}$ denote the \emph{vector-valued weighting} matrix. Note that $\bOm$ is a weight matrix that enables coordinate-wise weighting. Throughout the paper, we use $\bom$ and $\bOm$ to denote sample-wise and coordinate-wise weighting parameters, corresponding to scalar and vector gating strategies, respectively. Then given $\bOm$, we can similarly define
\begin{subequations}\label{eq:wpgd}
\begin{equation}
\bt_{\text{1}}^{\text{gd}}(\Pb_1, \Pb_2, \bOm) := \Pb_2 (\X \Pb_1 \odot \bOm)^\top \y \label{eq:wpgd:pred}
\end{equation} 
as one-step of (generalized) WPGD. Its corresponding prediction on a test query $\x$ is:
\begin{equation} 
\hat{y} = \x^\top \hat{\bt}, \quad \text{where} \quad \hat{\bt} = \bt_{\text{1}}^{\text{gd}}(\Pb_1, \Pb_2, \bOm).
\end{equation} 
\end{subequations}
We note that by removing the weighting matrix $\bOm$, \eqref{eq:wpgd} reduces to standard PGD (cf. \eqref{PGD pred}) and setting $\bOm=\bom\onebb_d^\top$ reduces to sample-wise WPGD (cf. \eqref{eqn:gd:wpgd-basic}).
% as given in \eqref{eqn:gd}.
\cite{li2024fine} has demonstrated that H3-like models implement one-step { \emph{sample-wise} WPGD}, and they focus on the shared-task distribution where $\bt_i \equiv \bt$ for all $i \in [n]$. In contrast, our work considers a more general data setting where tasks within an in-context prompt are not necessarily identical.  

We introduce the following model constructions under which we establish the equivalence between GLA (cf. \eqref{eq:GLA}) and WPGD (cf. \eqref{eq:wpgd}), where the weighting matrix is induced by the input data and the gating function. Inspired by prior works \citep{von2023transformers,ahn2024transformers}, we consider the following restricted attention matrices:
\begin{align}
\Wk &= \begin{bmatrix}
    \Pk & \zerobb \\
    \zerobb & 0
\end{bmatrix}, \quad
\Wq = \begin{bmatrix}
    \Pq & \zerobb \\
    \zerobb & 0
\end{bmatrix}, \quad \text{and} \quad
\Wv = \begin{bmatrix}
    \zerobb_{d\times d} & \zerobb \\
    \zerobb & 1
\end{bmatrix}, \label{att mtx res}
\end{align}
where $\Pk, \Pq \in \R^{d \times d}$. Note that the $(d+1, d+1)$-th entry of $\Wv$ is set to one for simplicity. More generally, this entry can take any nonzero value, e.g., $v \in \R$. Parameterizing $\Wq$ with $\Pq / v$ produces the same output as in \eqref{att mtx res}.
% In case of GLA, $\tGb$ will be given as a multiplication of data-dependent weights. Specifically, 
% We first introduce the following model constructions under which we establish the equivalence between GLA (c.f. \eqref{eq:GLA}) and WPGD (c.f. \eqref{eq:wpgd}) with the weighting matrix induced by the input data and the gating function. Inspired by previous works \citep{von2023transformers,ahn2024transformers}, we consider the following restricted attention matrices:
% \begin{align}\Wk=\begin{bmatrix}
%     \Pk^\top&\zerobb\\
%     \zerobb&0
% \end{bmatrix},\quad\Wq=\begin{bmatrix}
%     \Pq^\top&\zerobb\\\zerobb&0
% \end{bmatrix}\quad\text{and}\quad\Wv=\begin{bmatrix} \zerobb_{d\times d}&\zerobb\\\zerobb&1\end{bmatrix},\label{att mtx res}
% \end{align}
% % where $\Pk,\Pq\in\R^{d\times d}$. Here note that we set the $(d+1,d+1)$'th entry of $\Wv$ to be one for simplification. More generally, it can be any nonzero number, e.g., $v\in\R$. Then parameterizing $\Wq$ with $\Pq/v$ returns the same output as from \eqref{att mtx res}. 
% where $\Pk, \Pq \in \R^{d \times d}$. Note that the $(d+1, d+1)$-th entry of $\Wv$ is set to one for simplicity. More generally, this entry can take any nonzero value, e.g., $v \in \R$. Parameterizing $\Wq$ with $\Pq / v$ produces the same output as in \eqref{att mtx res}.


\begin{theorem}\label{thm:gla=wpgd} Recall \eqref{eq:GLA} with input sequence $\Z =[\z_1~~\dots~~\z_n~~\z_{n+1}]^\top$ defined in \eqref{input},  the gating  $G(\z_i)=\Gb_i\in\R^{(d+1)\times (d+1)}$, and outputs  $(\ob_{i})_{i=1}^{n+1}$. %Suppose that at time $i$, gating function has the form of $G(\z_i)=\Gb_i\in\R^{(d+1)\times (d+1)}$. 
Consider model construction in \eqref{att mtx res} and take the last coordinate of the last token output  denoted by $(\ob_{n+1})_{d+1}$ as a prediction. Then, we have % the single-layer GLA prediction (cf.~\eqref{eq:GLA})returns
\[
f_{\gla}(\Z):=(\ob_{n+1})_{d+1}%\ob_{n+1}^\top\hb
=\x^\top\hat\bt,\quad\textnormal{where}\quad\hat\bt=\bt_{\text{1}}^{\text{gd}}(\Pk,\Pq,\bOm).
\]
Here, $\bt_{\text{1}}^{\text{gd}}(\cdot)$ is a one-step WPGD feature predictor defined in \eqref{eq:wpgd:pred}; $\Pb_k$ and $\Pb_q$ correspond to attention weights following \eqref{att mtx res}; and
$\bOm=[\g_{1:n+1}~\cdots~\g_{n:n+1}]^\top\in\R^{n\times d}$, where $\g_{i:n+1},i\in[n]$ is given by
\begin{align}
\g_{i:n+1}:= {\g_{i+1}\odot \g_{i+2}\cdots \g_{n+1}} \in\R^d,\quad\textnormal{and}\quad\Gb_i=\begin{bmatrix}
    *&*\\
    \g_i^\top&*
\end{bmatrix}
.
\label{weighting}
\end{align}
\end{theorem}
Here and throughout, we use $*$ to fill the entries of the matrices that do not affect the final output. Based on the {model construction} in \eqref{att mtx res}, these entries can be assigned any value.


Observe that, crucially, since $\g_i$ is associated with $\z_i$, $\z_i$ influences the weighting of $\z_{j}$ {for all $j <i$}. We defer the proof of Theorem~\ref{thm:gla=wpgd} to the Appendix~\ref{app:1 layer}. It is noticeable that only $d$ of the total $(d+1)^2$ entries in each gating matrix $\Gb_i$ are useful due to the model construction presented in \eqref{att mtx res}.   However, if we relax the weight restriction, e.g., $\Wv=[\zerobb_{(d+1)\times d}~~\ub]^\top$, where $\ub\in\R^{d+1}$, then the weighting matrix $\bOm$ in Theorem~\ref{thm:gla=wpgd} is associated with all rows of the $\Gb_i$ matrices. We defer to Eqn. \eqref{eqn:allrow} and  the discussion in Appendix~\ref{app:1 layer}. % and Theorem~\ref{thm:gla optim vector}. 
%\da{do u mean this  \eqref{eqn:allrow}? can you clarify it?} \YL{I don't understand the comment. $\W_v$ is the value matrix.} 
\paragraph*{Capabilities of multi-layer GLA.} 
\citet{ahn2024transformers} demonstrated that, with appropriate construction, an $L$-layer linear attention model performs $L$ steps of PGD on the dataset $(\mathbf{x}_i, y_i)_{i=1}^n$ provided within the prompt. 
In Appendix~\ref{sec:multi layer}, we extend this analysis to multi-layer GLA and characterize the algorithmic class it can emulate. Importantly, \citet{ahn2024transformers} does not account for \emph{causal masking}, which is a fundamental aspect of multi-layer GLA due to its recurrent structure as described in \eqref{eq:GLA}. Our main result, Theorem~\ref{lemma:multi layer} in Appendix~\ref{sec:multi layer}, establishes that an $L$-layer GLA implements $L$ steps of WPGD, where the gradients are computed in a recurrent form.

\paragraph*{{GLA with scalar gating.}}

Theorem~\ref{thm:gla=wpgd} establishes a connection between one-layer GLA (cf.~\eqref{eq:GLA}) and one-step WPGD (cf.~\eqref{eq:wpgd}), where the weighting in WPGD corresponds to the gating $G(\z_i)=\Gb_i$ in GLA, as detailed in Theorem~\ref{thm:gla=wpgd}. Now let us consider the widely used types of gating functions, such as $\Gb_i=\bal_i\onebb^\top_{d+1}$ 
% \da{is it a matrix or vector? if it is a vector, i think it should be $\g_i=\bal_i\onebb^\top_{d+1}$ } 
\citep{yang2023gated,katsch2023gateloop,qin2024hgrn2,peng2024eagle} or $\Gb_i=\gamma_i\onebb_{(d+1),(d+1)}$ \citep{dao2024transformers,beck2024xlstm,peng2021random,sun2024you}, where $\bal_i\in\R^{d+1}$ and $\gamma_i\in\R$. In both cases, the gating matrices in \eqref{weighting} take the form of $\begin{bmatrix}
    *&*\\g_i\onebb_d^\top&*
\end{bmatrix}$ for some $g_i\in\R$, thus simplifying the predictor to a sample-wise WPGD, as given by 
\begin{align}
% \hat y:=\ob_{n+1,d+1}=
f_{\gla}(\Z)=\hat\bt^\top\x,\quad\textnormal{with}\quad\hat\bt=\Pb\X^\top(\bom\odot\y),\label{wpgd y}
\end{align}
where $\Pb=\Pq\Pk^\top$ and $\bom=[g_{1:n+1}~\cdots~g_{n:n+1}]^\top\in\R^n$. In the remainder, we will mostly focus on the one-layer GLA with scalar gating as presented in \eqref{wpgd y}. 
% \da{is it sample-wise similar to what we had below eqn (7). I think we need to use consistent notation.}
% Specifically, Section~\ref{sec:optim gd}

==> colm_sec/intro.tex <==
\section{Introduction}

The Transformer \citep{vaswani2017attention} has become the de facto standard for language modeling tasks. The key component of the Transformer is the self-attention mechanism, which computes softmax-based similarities between all token pairs. Despite its success, the self-attention mechanism has quadratic complexity with respect to sequence length, making it computationally expensive for long sequences. To address this issue, a growing body of work has proposed near-linear time approaches to sequence modeling. The initial approaches included linear attention and state-space models, both achieving $O(1)$ inference complexity per generated token, thanks to their recurrent form. While these initial architectures typically do not match softmax attention in performance, recent recurrent models such as Mamba~\citep{gu2023mamba,dao2024transformers}, mLSTM~\citep{beck2024xlstm}, GLA Transformer~\citep{yang2023gated}, and RWKV-6~\citep{peng2024eagle} achieve highly competitive results with the softmax Transformer. Notably, as highlighted in \citet{yang2023gated}, these architectures can be viewed as variants of \textit{gated linear attention} (GLA), which incorporates a gating mechanism within the recurrence of linear attention.
  

Given a sequence of tokens $(\z_i)_{i=1}^{n+1} \in \R^{d+1}$ and the associated query, key, and value embeddings $(\qb_i,\kb_i,\vb_i)_{i=1}^{n+1} \subset \mathbb{R}^{d+1}$, with $d+1$ being the embedding dimension\footnote{The sequence length and embedding dimension are set to \( n+1 \) and \( d+1 \) per the prompt definition in \eqref{input}.}, the GLA recurrence is given by
    % \da{I don't think ${\gla}(\Z)$ is a well-defined function or map. It also adds confusion with $f_{\gla}(\Z)$}
\begin{equation}\tag{GLA}
\label{eq:GLA}
\begin{split}    
&\Sb_{i} = \Gb_i \odot \Sb_{i-1} + \vb_i \kb_i^\top,\quad\text{and}\quad\ob_i = \Sb_{i} \qb_i, \quad   i  \in \left\{1,\ldots, n+1\right\}.
\end{split}
\end{equation}
% \begin{equation}\tag{GLA}
% \label{eq:GLA}
%     \begin{split}
%     &{\gla}(\Z)=[\ob_1,\ob_2, ~\cdots,~\ob_{n+1}]^\top\in\R^{(n+1)\times (d+1)}, \quad \text{where}\quad\\
%   &\ob_i = \Sb_{i} \qb_i, \quad\text{and}\quad\Sb_{i} = \Gb_i \odot \Sb_{i-1} + \vb_i \kb_i^\top,  \quad   i  \in \left\{1,\ldots, n+1\right\}.
%     \end{split}
% \end{equation}
Here, $\Sb_i \in \mathbb{R}^{(d+1) \times (d+1)}$ represents the \textit{2D state variable} with $\Sb_0 = \mathbf{0}$; $\ob_i \in \mathbb{R}^{d+1}$ represents the $i$th output token; and the \textit{gating variable} 
$\Gb_i := G(\z_i) \in \mathbb{R}^{(d+1) \times (d+1)}$ is applied to the state $\Sb_{i-1}$ through the Hadamard product $\odot$ and $G$ represents the gating function. When $\Gb_i$ is a matrix of all ones, \eqref{eq:GLA} reduces to causal linear attention~\citep{katharopoulos2020transformers}.


The central objective of this work is to enhance the mathematical understanding of the GLA mechanism. In-context learning (ICL), one of the most remarkable features of modern sequence models, provides a powerful framework to achieve this aim. ICL refers to the ability of a sequence model to implicitly infer functional relationships from the demonstrations provided in its context window \citep{brown2020language,min2022rethinking}. It is inherently related to the model's ability to emulate learning algorithms. Notably, ICL has been a major topic of empirical and theoretical interest in recent years.  More specifically, a series of works have examined the approximation and optimization characteristics of linear attention, and have provably connected linear attention to the preconditioned gradient descent algorithm \citep{von2023transformers,ahn2024transformers,zhang2024trained}. Given that the GLA recurrence in \eqref{eq:GLA} has a richer design space, this leads us to ask: 
%
%
\begin{quote}
\begin{center}    
\textit{{\color{black}What learning algorithm does GLA emulate in ICL?%\\
% How does its optimization landscape behave in multi-task settings?
}}
\end{center}
\end{quote}
%
%
\noindent\textbf{Contributions:} The \eqref{eq:GLA} recurrence enables the sequence model to weight past information in a data-dependent manner through the gating mechanism $(\Gb_i)_{i=1}^{n}$. Building on this observation, we demonstrate that a GLA model can implement a \emph{data-dependent Weighted Preconditioned Gradient Descent (WPGD)} algorithm. Specifically, a one-step WPGD with scalar gating, where all entries of $\Gb_i$ are identical, is described by the prediction:
\begin{align}
\hat{y} = \x^\top \Pb \X^\top(\y \odot \bom).\label{wpgd}
\end{align}
Here, $\X \in \R^{n \times d}$ is the input feature matrix; $\y \in \R^n$ is the associated label vector; $\x \in \R^d$ represents the test/query input to predict; $\Pb \in \R^{d \times d}$ is the preconditioning matrix; and $\bom \in \R^n$ weights the individual samples. When $\bom$ is fixed, we drop ``data-dependent'' and simply refer to this algorithm as the WPGD algorithm. However, for GLA, $\bom$
% := \bom(\X, \y)$ 
% \da{there is no $\bom(\X, \y)$. can we remove it? } 
depends on the data through recursive multiplication of the gating variables. Building on this formalism, we make the following specific contributions:
\begin{enumerate}[label=$\diamond$]
\item \textbf{ICL capabilities of GLA (\S\ref{sec plain wpgd}):} Through constructive arguments, we demonstrate that a multilayer GLA model can implement data-dependent WPGD iterations, with weights induced by the gating function. This construction sheds light on the role of causal masking and the expressivity distinctions between scalar- and vector-valued gating functions.
\item \textbf{Landscape of {{one}}-step WPGD (\S\ref{sec:optim gd}):} The GLA$\Leftrightarrow$WPGD connection motivates us to ask: \emph{How does WPGD weigh demonstrations in terms of their relevance to the query?} To address this, we study the fundamental problem of learning an optimal WPGD algorithm: Given a tuple $(\X,\y,\x,y)\sim \Dc$, with $y\in\R$ being the label associated with the query, we investigate the population risk minimization:
\begin{equation}\label{eqn:wpgd:risk}
\begin{split}
&\Lc_\wpgd^\st := \min_{\Pb {\in \mathbb{R}^{d \times d}},\bom \in \R^n}~\Lc_\wpgd(\Pb,\bom), ~\\
&\text{where}~~\Lc_\wpgd(\Pb,\bom)=\E_{\Dc}\left[\left(y-\x^\top \Pb \X^\top(\y\odot\bom)\right)^2\right].
\end{split}
\end{equation}
As our primary mathematical contribution, we characterize the loss landscape under a general multitask data setting, where the tasks associated with the demonstrations $(\X,\y)$ have varying degrees of correlation to the target task $(\x,y)$. We carefully analyze this loss landscape and show that, under mild conditions, there is a unique global minimum $(\Pb,\bom)$ up to scaling invariance, and the associated WPGD algorithm is also unique.

\item \textbf{Loss landscape of {{one}}-layer GLA (\S\ref{gla sec}):} The landscape is highly intricate due to the recursively multiplied gating variables. We show that learning the optimal GLA layer can be connected to solving \eqref{eqn:wpgd:risk} with a constraint $\bom\in\Wc$, where the restriction $\Wc$ is induced by the choice of gating function and input space. Solidifying this connection, we introduce a multitask prompt model under which we characterize the loss landscape of GLA and the influence of task correlations. Our analysis and experiments reveal insightful distinctions between linear attention, GLA with scalar gating, and GLA with vector-valued gating.
\end{enumerate}


==> colm_sec/loss_landscape_iid.tex <==
\section{Additional corollaries}
In this section, we present additional corollaries derived from Section~\ref{sec:optim gd}  under the assumption that $\bSi=\Iden$.
\paragraph*{Loss landscape of WPGD.}Following Theorems~\ref{thm:station:wpgd} and \ref{thm:unique:wpgd} in Section~\ref{sec:optim gd}, by setting the data covariance (cf. Definition~\ref{def:multitask}) to \(\bSi = \Iden\), we directly obtain the following corollary on the optimal loss for the WPGD problem defined in \eqref{eqn:wpgd:risk}.


\begin{corollary}\label{coroll:unique}
Suppose $\bSi = \Iden$. Then, $\Delta_{\bSi} = 0$, satisfying Condition~\eqref{eqn:gap:cond}, and we have $h_2(\gamma^\star) = \frac{1}{d + \sigma^2 + 1}$, which yields
%\begin{equation}%\label{eqn:opt:obj}
$\Pb^\star = \Iden$ {and} $\bom^\star = ( \Rb + (d + \sigma^2 + 1)\Iden )^{-1} \rb$.
%\end{equation}
Thus, the optimal risk $\Lc^\st_\wpgd$ defined in \eqref{eqn:wpgd:risk} is given by
\begin{equation}
    \Lc_\wpgd^
    \st= d+\sigma^2  -  d \cdot \rb^\top\left( \Rb + (d + \sigma^2 + 1)\Iden \right)^{-1} \rb.\label{optim wpgd risk}
\end{equation}
\end{corollary}

\paragraph*{Loss landscape of One-layer linear attention.} Given the fact that linear attention is equivalent to \eqref{eq:GLA} when implemented with all ones gating, that is, $\Gb_i\equiv\onebb$, we derive the following corollary. Consider training a standard single-layer linear attention, i.e.,  by setting $\Gb_i\equiv\onebb$ in \eqref{eq:GLA}, and let $f_{\att}(\Z)$ be its prediction. Let  $\Lc_\att^\st$ be the corresponding optimal risk following \eqref{eqn:gla:risk}.  
\begin{corollary}\label{corol:att}
Consider a single-layer linear attention following model construction in \eqref{att mtx res} and let linear data as given in Definition~\ref{def:multitask}. Let $\Rb$ and $\rb$ be the corresponding correlation matrix and vector as defined in Definition~\ref{corr task def}. 
Suppose $\bSi=\Iden$. Then, the optimal risk obeys
\begin{align}
\Lc^\st_\att:=\min_{\Pb\in\R^{d\times d}}\Lc_\wpgd(\Pb,\bom=\onebb)=d+\sigma^2 - \frac{d(\onebb^\top \rb)^2}{n(d+\sigma^2+1) + \onebb^\top \Rb \onebb}.\label{optim att risk}
\end{align}
% \rebuttal{
% Additionally, recalling the $\Lc^\st_\wpgd$ defined in \eqref{eqn:wpgd:risk} and Corollary~\ref{coroll:unique}, we obtain
% \[
% \Lc^\st_\att-\Lc^\st_\wpgd=d \cdot \rb^\top\left(\Rb_+^{-1} -\frac{\onebb\onebb^\top}{\onebb^\top \Rb_+ \onebb}\right)\rb\geq0\quad\text{where}\quad\Rb_+:= \Rb + (d + \sigma^2 + 1)\Iden. 
% \]
% }
\end{corollary}

% \begin{corollary}\label{corol:att vs gla}
% Consider the same setting as discussed in Corollary~\ref{corol:att}, and suppose Assumption~\ref{assum delimiter gate} holds, it satisfies that $\Lc^\st_\att\geq\Lc^\st_\gla$. Additionally, suppose Assumption~\ref{assum order} holds, we obtain
% \[
% \Lc^\st_\att-\Lc^\st_\gla=d \cdot \rb^\top\left(\Rb_+^{-1} -\frac{\onebb\onebb^\top}{\onebb^\top \Rb_+ \onebb}\right)\rb\geq0\quad\text{where}\quad\Rb_+:= \Rb + (d + \sigma^2 + 1)\Iden. 
% \]
% \end{corollary}
% \begin{comment}
\begin{corollary}[Benefit of Gating]\label{corol:att vs gla}
Consider the same setting as discussed in Corollary~\ref{corol:att}, and suppose Assumption~\ref{assum delimiter gate} holds. Then, we have that $\Lc^\st_\att \geq \Lc^\st_\gla$. Additionally, if Assumption~\ref{assum order} holds, we obtain
\[
\Lc^\st_\att - \Lc^\st_\gla = d \cdot \rb^\top\left(\Rb_+^{-1} - \frac{\onebb\onebb^\top}{\onebb^\top \Rb_+ \onebb}\right)\rb \geq 0, \quad \textnormal{where}\quad   \Rb_+ := \Rb + \left(d + \sigma^2 + 1\right)\Iden.
\]
\end{corollary}
The proof of this corollary is directly from \eqref{optim wpgd risk}, \eqref{gla=wpgd} and \eqref{optim att risk}.
% \end{comment}
In the Figure~\ref{fig:k=2}, blue solid curves represent the linear attention results
 and blue dashed are the theory curves following \eqref{optim att risk}. The two curves are aligned in all the subfigures, which validate our Corollary~\ref{corol:att}. More implementation details are deferred to Appendix~\ref{sec:exp}.

==> colm_sec/multi_layer.tex <==
\section{Capabilities of multi-layer GLA}\label{sec:multi layer}
% Previous work 
\citet{ahn2024transformers} demonstrated that, with appropriate construction, an $L$-layer linear {attention model}
% \asrnote{Is it `transformer' or `attention'?}
performs $L$-step preconditioned GD on the dataset $(\x_i, y_i)_{i=1}^n$ provided within the prompt. 
% \update{However, their analysis did not account for the causal mask, which is commonly used in practice.}
In this work, we study multi-layer GLA and analyze the associated algorithm class it can emulate. 
% \update{Note that, given the recurrent formulation in \eqref{eq:GLA}, the causal mask is inherently incorporated.}
{It is worth mentioning that \citet{ahn2024transformers} does not consider \textit{causal masking} which is integral to multilayer GLA due to its recurrent nature described in \eqref{eq:GLA}. Our analysis will capture the impact of gating and causal mask through $n$ separate GD trajectories that are coupled.}


\paragraph*{Multi-layer GLA.} For any input prompt $\Z\in\R^{(n+1)\times(d+1)}$, let $\gla(\Z):=[\ob_1~~\ob_2~~\cdots~~\ob_{n+1}]^{\top}\in\R^{(n+1)\times(d+1)}$ denote its GLA output, as defined in \eqref{eq:GLA}.  
We consider an $L$-layer GLA model as follows:  
For each layer $\ell\in[L]$, let $\Z_\ell$ denote its input, where we set $\Z_1=\Z$, and let $\W_{k,\ell},\W_{q,\ell},\W_{v,\ell}$ denote the key, query, and value matrices for layer $\ell$, respectively. After applying a residual connection, the input of the $\ell$-th layer is given by
\begin{align}\label{gla multi}
    \Z_\ell:=\Z_{\ell-1}+\gla_{\ell-1}(\Z_{\ell-1}). %\tag{$L$-GLA}
\end{align}
Here, $\gla_\ell(\cdot)$ denotes the output of the $\ell$-th GLA layer, associated with the attention matrices $(\W_{q,\ell},\W_{k,\ell},\W_{v,\ell})$ for all $\ell\in[L]$. In the following, we focus on the $(d+1)$-th entry of each token's output at each layer (after the residual connection), denoted by $o_{i,\ell} := [\Z_\ell+\gla_\ell(\Z_\ell)]_{i,d+1}$ for all $i \in [n+1]$ and $\ell\in[L]$.
% Consider an $L$-layer GLA model. For each layer $\ell\in[L]$, let $\Z_\ell$ and $\Ob_\ell$ denote the input and output of the $\ell$'th layer. In practice, residual connections are commonly applied \citep{vaswani2017attention}. Hence, we define the updated output of the $\ell$'th layer (after applying the residual connection) as $\tilde\Ob_\ell := \Z_\ell + \Ob_\ell$. Note that $\tilde\Ob_\ell$ also serves as the input to the $(\ell+1)$'th layer, i.e., $\Z_{\ell+1} = \tilde\Ob_\ell$. In the following, we focus on $(d+1)$'th entries of each token's output at each layer, denoted by $\tilde o_{i,\ell}:=(\tilde\Ob_\ell)_{i,d+1}$ for $i \in [n+1],\ell\in[L]$. 

\begin{theorem}\label{lemma:multi layer}
% \da{should we use \eqref{gla multi} in the statment of the theorem? Have you used it somwhere?}
Consider an $L$-layer GLA  defined in \eqref{gla multi}, %each layer follows the weight construction specified in \eqref{att mtx res}. Let 
where  $\W_{k,\ell}$, $\W_{q,\ell}$ in the $\ell$'th layer parameterized by $\Pkl, -\Pql \in \R^{d \times d}$, for all  $\ell \in [L]$ following \eqref{att mtx res}. Let the gating be a function of the features, e.g., $\Gb_i =G(\x_i)$, and define $\bOm$ as in Theorem~\ref{thm:gla=wpgd}. 
% Consider an $L$-layer GLA with residual connections, where $\Wk$ and $\Wq$ in the $\ell$'th layer are parameterized by $\Pkl, \Pql \in \R^{d \times d}$, following \eqref{att mtx res}, for $\ell \in [L]$. Let the gating be a function of the features, e.g., $\Gb_i = g(\x_i)$, and let $\bOm$ be defined as in Theorem~\ref{thm:gla=wpgd}. 
Additionally, denote the masking as $\M_i = \begin{bmatrix}
    \Iden_i & \zerobb\\
    \zerobb & \zerobb
\end{bmatrix} \in \R^{n \times n}$, and  let $\hat\bt_0=\btm{i}{0} = \zerobb$ for all $i \in [n]$. Recall that $ o_{i,\ell}$ for all  $i \in [n+1]$ and $\ell\in[L]$ stands for the last entry of the $i$'th token output at the $\ell$'th layer. We have 
\begin{itemize}
    \item For all $i \leq n$, $ o_{i,\ell} = y_i - \x_i^\top \bt_{i,\ell}$, where $\bt_{i,\ell} = \bt_{i,\ell-1} {-\Pql} \left(\nabla_{i,\ell} \oslash \g_{i:n+1}\right)$;
    \item $ o_{n+1,\ell} = -\x^\top \hat\bt_{\ell}$, where $\hat\bt_{\ell} = (1 - \alpha_{\ell}) \hat\bt_{\ell-1} -\Pql \left(\nabla_{n,\ell} \oslash \g_{n+1}\right)$, and $\alpha_\ell = \x^\top \Pql \Pkl^\top \x$.
\end{itemize}
Here, letting $\B_{\ell} = [\btm{1}{\ell}~\cdots~\btm{n}{\ell}]^\top$, $\X_{\ell} = \X\Pb_{k,\ell} \odot \bOm$, 
and $\y_\ell = \textnormal{diag}(\X\B_\ell^\top)$, we define 
\[
\nabla_{i,\ell} = \X_{\ell}^\top \M_i \left(\y_\ell-\y\right).
\]
\end{theorem}

We defer the proof of Theorem~\ref{lemma:multi layer} to the Appendix~\ref{app:multi layer}. Theorem~\ref{lemma:multi layer} states that $L$-layer GLA \eqref{gla multi}  implements $L$ steps of WPGD with gradient in a recurrent form and additional weight decay $\alpha_\ell$. To recap, given data $(\X, \y)$ and prediction $\hat\bt$, the gradient with respect to the squared loss takes the form $\X^\top(\X\hat\bt - \y)$, up to some constant $c$. In comparison, $\Pql\left(\nabla_{i,\ell}\oslash\g_{i:n+1}\right)$ similarly acts as a gradient but incorporates layer-wise feature preconditioners ($\Pql, \Pkl$), data weighting ($\bOm$), and causality ($\g_{i:n+1}, \M_i$). Here, $\M_i$ represents causal masking, ensuring that at time $i$, only inputs from $j \leq i$ are used for prediction. Notably, the recurrent structure of GLA allows the gating mechanism to apply context-dependent weighting strategies.


To simplify the theorem statement, we assume that the gating function depends only on the input feature, e.g., $\Gb_i = G(\x_i)$, ensuring that the corresponding data-dependent weighting is uniform across all layers. This assumption is included solely for clarity in the theorem statement, and if the gating function varies across layers or depends on the entire $(d+1)$-dimensional token rather than just the feature $\x_i$, each layer has its own gating $\bOm_\ell$ and $\X_\ell=\X\Pkl\odot\bOm_{\ell}$. Note that our inclusion of the additional term $\alpha_\ell$ captures the influence of the last token's output on the next layer’s prediction. Based on the above $L$-layer GLA result, we have the following corollary for multi-layer linear attention network with causal mask in each layer.

% \begin{corollary}
%     Consider an $L$-layer linear attention model with causal mask and residual connection in each layer. Let $\ell$'th layer be parameterized by $\Pql,\Pkl$ as in \eqref{att mtx res} and define $\Pb_\ell:=\yl{-\Pql\Pkl^\top}$, $\ell\in[L]$. Let $\hat\bt_0,\btm{i}{0}=\zerobb$ for $i\in[n]$. Then, the $(d+1)$'th entry of the $i$'th token of the $\ell$'th layer outputs satisfies:
% \begin{itemize}
%     \item For~$i\leq n$, $\tilde o_{i,\ell}=y_i-\x_i^\top\bt_{i,\ell}$ where $\bt_{i,\ell}=\bt_{i,\ell-1}\yl{-\Pl}\nabla_{i,\ell}$,
%     \item $\tilde o_{n+1,\ell}=-\x^\top\hat\bt_{\ell}$ where $\hat\bt_{\ell}=(1+\alpha_{\ell})\hat\bt_{\ell-1}\yl{-\Pl}\nabla_{n,\ell}$ and $\alpha_\ell=\x^\top\Pl\x$.
% \end{itemize}
% Here, we define $\nabla_{i,\ell}=\X^\top\M_i\left(\hat\y_{\ell}-\y\right)$ with $\hat\y_\ell,\M_i$ following the same definitions as in Theorem~\ref{lemma:multi layer}.
% \end{corollary}


\begin{corollary}\label{corol multi}
    Consider an $L$-layer linear attention model with causal mask and residual connection in each layer. Let $\ell$'th layer follows the weight construction in \eqref{att mtx res} with $\W_{k,\ell},\W_{q,\ell}$ parameterized by $\Pkl,{-\Pql}$ as in Theorem~\ref{lemma:multi layer} and define $\Pb_\ell:={\Pql\Pkl^\top}$, for $\ell\in[L]$. Let $\hat\bt_0=\zerobb$. Then, the $(d+1)$'th entry of the last token output of each layer satisfies:
    \begin{align*}
         o_{n+1,\ell}=-\x^\top\hat\bt_{\ell}, \quad \text{where}\quad \hat\bt_{\ell}=(1-\alpha_{\ell})\hat\bt_{\ell-1}{-\Pl}\X^\top(\y_{\ell}-\y).
    \end{align*}
Here, we define $\alpha_\ell=\x^\top\Pl\x$ and $\y_\ell$ follows the same definition as in Theorem~\ref{lemma:multi layer}.
\end{corollary}

Note that Corollary~\ref{corol multi} generalizes \cite[Lemma 1]{ahn2024transformers} by extending it to causal attention. When considering full attention (i.e., without applying the causal mask), we have $\y_\ell = \X\hat\bt_\ell$, and the expression $\X^\top(\y_\ell-\y) = \X^\top(\X\hat\bt_\ell - \y)$ corresponds to the standard gradient of the squared loss. Furthermore, if we disregard the impact of the last token (e.g., by incorporating the matrix $M$ as in Eq. (3) of \cite{ahn2024transformers}), then $\alpha_\ell = 0$. These results are also consistent with \cite{ding2023causallm}, which demonstrate that causal masking limits convergence by introducing sequence biases, akin to online gradient descent with non-decaying step sizes.
 

Our theoretical results in Theorem \ref{lemma:multi layer} focus on multi-layer GLA without Multi-Layer Perceptron (MLP) layers to isolate and analyze the effects of the gating mechanism. However, MLP layers, a key component of standard Transformers, facilitate further nonlinear feature transformations and interactions, potentially enhancing GLA's expressive power. Future work could explore the theoretical foundations of integrating MLPs into GLA and analyze the optimization landscape of general gated attention models, aligning them more closely with conventional Transformer architectures \citep{gu2023mamba,dao2024transformers,peng2024eagle}.




==> colm_sec/setup.tex <==
\section{Problem setup}\label{sec:setup}
\emph{Notations.}
$\mathbb{R}^d$ is the $d$-dimensional real space, with $\mathbb{R}^d_{+}$ and $\mathbb{R}^d_{++}$ as its positive and strictly positive orthants. The set $[n]$ denotes $\{1, \dots, n\}$. Bold letters, e.g., $\ab$ and $\A$, represent vectors and matrices. The identity matrix of size $n$ is denoted by $\Iden_n$. The symbols $\onebb$ and $\zerobb$ denote the all-one and all-zero vectors or matrices of proper size, such as $\onebb_d \in \mathbb{R}^d$ and $\onebb_{d\times d} \in \mathbb{R}^{d\times d}$. The subscript is omitted when the dimension is clear from the context. The Gaussian distribution with mean $\bmu$ and covariance $\bSi$ is written as $\mathcal{N}(\bmu,\bSi)$. The Hadamard product (element-wise multiplication) is denoted by $\odot$, and Hadamard division (element-wise division) is denoted by $\oslash$. Given any $\ab_{i+1}, \dots, \ab_j \in \mathbb{R}^d$, we define $\ab_{i:j} = \ab_{i+1} \odot \cdots \odot \ab_j$ for $i < j$, and $\ab_{i:i} = \onebb_d$.


The objective of this work is to develop a theoretical understanding of GLA through ICL. The optimization landscape of standard linear attention has been a topic of significant interest in the {ICL} literature~\citep{ahn2024transformers,li2024fine}. Following these works, we consider the input prompt
\begin{align}
\Z=[\z_1~~~\dots~~~\z_n~~~\z_{n+1}]^\top=
\begin{bmatrix}
\x_1 & \dots & \x_n & \x_{n+1} \\
y_1 & \dots & y_n & 0
\end{bmatrix}^\top
\in\R^{(n+1)\times(d+1)},\label{input}
\end{align}
where tokens encode the input-label pairs $(\x_i,y_i)_{i=1}^{n}\subset\R^d\times\R$. 

We aim to enable ICL by training a sequence model $F: \R^{(n+1) \times (d+1)} \to \R
$ that predicts the label $y:=y_{n+1}$ associated with the query $\x:=\x_{n+1}$. 
This model will utilize the demonstrations $(\x_i,y_i)_{i=1}^n$ to infer the mapping between $\x$ and $y$. Assuming that the data is distributed as $(y,\Z)\sim \Dc$, the ICL objective is defined as
\begin{align}
\Lc(F)=\E_{\Dc}\left[\left(y-F(\Z)\right)^2\right].\label{ICL loss}
\end{align}

\paragraph*{Linear attention and shared-task distribution.}Central to our paper is the choice of the function class $F$. When $F$ is a linear attention model, 
the prediction $\hat y_F:=F(\Z)$ takes the form  
% \da{can we just clearly mention $F(\Z) = \z_{n+1}^\top \W_q \W_k^\top   \Z^\top \Z \W_v \h$? }
% \begin{align*}
$\hat{y}_{F} = \z_{n+1}^\top \W_q \W_k^\top   \Z^\top \Z \W_v \h$,    
% \end{align*}
where $\W_{k}, \W_{q}, \W_{v} \in \mathbb{R}^{(d+1) \times (d+1)}$ are attention parameters, and $\h \in \mathbb{R}^{d+1}$ is the linear prediction head. 
%

We assume that the in-context input-label pairs follow a \emph{shared-task distribution}, where $\bt \sim \mathcal{N}(\zerobb, \bSi_\bt)$, $\x_i$ are i.i.d. with $\x_i \sim \mathcal{N}(\zerobb, \bSi_{\x})$, and $y_i \sim \mathcal{N}(\bt^\top \x_i, \sigma^2)$, where $\sigma \geq 0$ represents the noise level.  Under this shared-task distribution, it is shown  \citep{von2023transformers,ahn2024transformers,zhang2024trained}  that the optimal one-layer linear attention prediction coincides with the one-step optimal preconditioned gradient descent (PGD). In particular, considering the data distribution discussed above, we have 
\begin{align}\label{PGD pred}
\hat y_F=\x^\top\hat\bt, \quad\text{where}\quad \hat\bt = \Pb^\star\X^\top \y,
\end{align}
and
\begin{align}
\Pb^\star:=\argmin_{\Pb \in \mathbb{R}^{d \times d}}~\E\left[\left(y-\x^\top \Pb\X^\top \y\right)^2\right]~~\text{with}~~ \X:= \begin{bmatrix} \x_1~\cdots~\x_n\end{bmatrix}^\top ~~\text{and}~~ \y:=\begin{bmatrix}y_1~\cdots~y_n\end{bmatrix}^\top.\label{PGD loss}
\end{align}
% {\color{magenta} what is $\Dc$? same as eqn 4 or is it Gaussian? }

\paragraph*{Linear attention and gating.} 
Given the input prompt $\Z$ as in \eqref{input}, let $(\qb_i, \kb_i,\vb_i)= (\W_q^\top\z_i, \W_k^\top\z_i,\W_v^\top\z_i)$ be the corresponding query, key,
and value embeddings.   The output of \textit{causal} linear attention at time $i$ can be computed {using \eqref{eq:GLA} with $\Gb_i = \onebb$}.  This recurrent form implies that linear attention has $O(d^2)$ cost, that is independent of sequence length $n$, to generate per-token. 
% As presented in \eqref{eq:GLA}, 
GLA follows the same structure as linear attention but with a gating mechanism {(i.e., $\Gb_i \neq \onebb$)}, which equips the model with the option to pass or supress the history.  As discussed in \cite{yang2023gated}, the different choices of the gating function correspond to different popular recurrent architectures such as Mamba \citep{gu2023mamba}, Mamba2 \citep{dao2024transformers}, RWKV \citep{peng2024eagle}, etc. 


We will show that GLA can weigh the context window through gating, thus, its capabilities are linked to the WPGD algorithm described in \eqref{eq:wpgd}. This will in turn facilitate GLA to effectively learn \emph{multitask prompt distributions} described by $y_i\sim\Nn(\bt_i^\top\x_i,\sigma^2)$ with $\bt_i$'s not necessarily identical. 

==> colm_sec/wpgd.tex <==
\section{Optimization landscape of WPGD}\label{sec:optim gd}
%
In this section, we explore the problem of learning the optimal {sample-wise WPGD} algorithm described in \eqref{wpgd y}, a key step leading to our analysis of GLA. The problem is as follows. Recap from \eqref{PGD loss} that we are given the tuple $(\x, y, \X, \y) \sim \Dc$, where $\X \in \R^{n \times d}$ is the input matrix, $\y \in \R^n$ is the label vector, $\x \in \R^d$ is the query, and $y \in \R$ is its associated label. The goal is to use $\X, \y$ to predict $y$ given $\x$ via the one-step WPGD prediction $\hat{y} = \x^\top \hat{\bt}$, with $\hat{\bt}$ as in \eqref{wpgd y}. The algorithm learning problem is given by \eqref{eqn:wpgd:risk} which minimizes the WPGD risk $\E_{\Dc}[\left(y-\x^\top \Pb \X(\bom \odot \y)\right)^2]$.

Prior research \citep{mahankali2023one,li2024fine,ahn2024transformers} has studied the problem of learning PGD when input-label pairs follow an i.i.d. distribution. It is worth noting that while \cite{li2024fine} establishes a connection between H3-like models and \eqref{wpgd y} similar to ours, their work assumes that the optimal $\bom$ consists of all ones and does not specifically explore the optimization landscape of $\bom$ when in-context samples are not generated from the same task vector $\bt$.  
Departing from this, we introduce a realistic model where each input-label pair is allowed to come from a distinct task.

\begin{definition}[Correlated Task Model] \label{corr task def} Suppose $\bt_i\in\R^d\sim \Nn(0,\Iden)$ are jointly Gaussian for all $i\in[n+1]$.  Define 
% the pairwise correlations $r_{ij}=\E[\bt_i^\top\bt_j]/d$ for $i,j\in[n+1]$, and \YL{We don't need to define $r_{ij}$ here}%\vspace{-10pt}
\begin{align}\label{eqn:Randr}
\bt:=\bt_{n+1},\quad \B:=[\bt_1~\dots~\bt_n]^\top,\quad \Rb:=\frac{1}{d}\E[\B\B^\top],\quad \textnormal{and}\quad \rb:=\frac{1}{d}\E[\B\bt].    
\end{align}
%Additionally, for any $i,j\in[n+1]$, $\bt_i-r_{ij}\bt_j$ is independent of $\bt_j$.
\end{definition}
% {\color{magenta}
% \begin{definition}[Correlated Task Model] \label{corr task def} Suppose $\bt_i\in\R^d\sim \Nn(0,\Iden)$ are jointly Gaussian for $i\in[n+1]$. Define  the pairwise correlations $r_{ij}=\E[\bt_i^\top\bt_j]/d$ for $i,j\in[n+1]$, and 
% \begin{align}\label{eqn:Randr}
% \bt:=\bt_{n+1},\quad \B=[\bt_1~\dots~\bt_n]^\top,\quad \Rb=[r_{ij}]_{i,j\in[n]},\quad\textnormal{and}\quad \rb= [r_{i,n+1}]_{i\in[n]}. 
% \end{align}
% \end{definition}
%}
Note that in \eqref{eqn:Randr}, we have $\Rb \in \R^{n \times n}$  and $\rb \in \R^n$, with normalization ensuring that the entries of $\Rb$ and $\rb$ lie in the range $[-1,1]$, corresponding to correlation coefficients. Further, due to the joint Gaussian nature of the tasks, for any $i,j\in[n+1]$, the residual $\bt_i-r_{ij}\bt_j$ is independent of $\bt_j$.
%
\begin{definition}[Multitask Distribution]\label{def:multitask}
Let $(\bt_i)_{i=1}^{n+1}$ be drawn according to the correlated task model of Definition~\ref{corr task def}, $(\x_i)_{i=1}^{n+1}\in\R^d$ be i.i.d. with $\x_i\sim\Nn(0,\bSi)$, and $y_i\sim\Nn(\x_i^\top\bt_i,\sigma^2)$ for all $i\in[n+1]$.
\end{definition}
% \begin{definition}[Multitask Distribution] 
% \label{def:multitask}
% Let $(\bt_i)_{i=1}^{n+1}$ be drawn according to the correlated task model given in Definition~\ref{corr task def}. Let $(\x_i)_{i=1}^{n+1} \in \R^d$ be i.i.d. random variables with $\x_i \sim \Nn(0, \bSi)$. For each $i \in [n+1]$, $y_i$ are generated as $y_i \sim \Nn(\x_i^\top \bt_i, \sigma^2)$.
% \end{definition}
%
%
\begin{definition}
Let the eigen decompositions of $\bSi$ and $\Rb$ be denoted by 
$\bSi = \Ub \textnormal{diag}(\s) \Ub^\top$ and $\Rb = \Eb \textnormal{diag}(\bla) \Eb^\top$, 
where $\s = [s_1~ \cdots~ s_d]^\top \in \R^d_{++}$ and $\bla = [\lambda_1~\cdots~ \lambda_n]^\top \in \R_{+}^n$. Let $s_{\min}$ and $s_{\max}$ denote the smallest and largest eigenvalues of $\bSi$, respectively. Further, let $\lambda_{\min}$ and $\lambda_{\max}$ denote the \textit{nonzero} smallest and largest eigenvalues of $\Rb$. Define the effective spectral gap of $\bSi$ and $\Rb$, respectively, as
\begin{align}\label{eqn:spec:gap}
\Delta_{\bSi} := s_{\max}- s_{\min}, \quad\textnormal{and}  \quad \Delta_{\Rb} := \lambda_{\max}-\lambda_{\min}. 
\end{align}
\end{definition}


\begin{assumption}\label{assum:rb:in:eigenspace}
{The correlation vector $\rb$ from \eqref{eqn:Randr} lies in the range of $\Eb$}, i.e., $\rb = \Eb \ab$ for some nonzero  $\ab = [a_1~ \cdots~ a_n]^\top \in \R^n$. 
\end{assumption}

Assumption~\ref{assum:rb:in:eigenspace} essentially ensures that $\rb$ (representing the correlations between in-context tasks) can be expressed as a linear transformation of a vector \(\ab \) with at least one nonzero value. {Note that since $\rb$ lies in the range of the eigenvector matrix $\Eb$, it also lies in the range of $\Rb$ defined in \eqref{eqn:Randr}}. This guarantees that the correlation structure is non-degenerate, meaning that all elements of \( \rb \) are influenced by meaningful correlations. Assumption~\ref{assum:rb:in:eigenspace} avoids trivial cases where there are no correlations between tasks. By requiring at least one nonzero element in \( \ab \), the assumption ensures that the tasks are interrelated.

The following theorem characterizes the stationary points $(\Pb, \bom)$ of the WPGD objective \eqref{eqn:wpgd:risk}.
%
\begin{theorem}\label{thm:station:wpgd}
Consider independent linear data as described in Definition~\ref{def:multitask}. Suppose Assumption~\ref{assum:rb:in:eigenspace} on the correlation vector $\rb$ holds. Define the functions $h_1: \mathbb{R}_{+} \to \mathbb{R}_{+}$ and $h_2: [1, \infty) \to \mathbb{R}_{+}$ as
\begin{subequations}
\begin{align}
    h_1(\bar{\gamma}) &:= \left(\sum_{i=1}^n \frac{\lambda_i a_i^2}{ \left(1 + \lambda_i \bar{\gamma} \right)^2}\right) \left( \sum_{i=1}^n \frac{a_i^2}{\left(1 + \lambda_i \bar{\gamma} \right)^2} \right)^{-1}, \label{func:h} \\
    h_2(\gamma) &:= \left(1+ M\left(\sum_{i=1}^d \frac{s_i^2}{(M + s_i \gamma)^2}\right)\left(\sum_{i=1}^d \frac{s_i^3}{(M +  s_i \gamma )^2}\right)^{-1} \right)^{-1}, \label{func:g}
\end{align}
\end{subequations}
where $\{s_i\}_{i=1}^d$ and $\{\lambda_i\}_{i=1}^n$ are the eigenvalues of $\bSi$ and $\Rb$, respectively; $\{a_i\}_{i=1}^n$ are given in Assumption~\ref{assum:rb:in:eigenspace}; and $M = \sigma^2 + \sum_{i=1}^d s_i$.


%where $h$ and $g$ are defined in terms of the eigenvalues $\lambda_i$ and $s_i$, respectively.
The risk function $\Lc_{\wpgd}(\Pb, \bom)$ in \eqref{eqn:wpgd:risk} has a stationary point $(\Pb^\star, \bom^\star)$, up to rescaling, defined as
\begin{align}\label{eqn:pstar_and_wstar}
    \Pb^\star &= \bSi^{-\frac{1}{2}} \left( \frac{\gamma^\star }{M} \cdot \bSi + \Iden \right)^{-1} \bSi^{-\frac{1}{2}}, \quad \textnormal{and} \quad \bom^\star = \left( h_2(\gamma^\star) \cdot \Rb + \Iden \right)^{-1} \rb,
\end{align}
where $\gamma^\star$ is a fixed point of composite function \( h_1(h_2(\gamma))+1\).
\end{theorem}

Theorem~\ref{thm:station:wpgd} characterizes the stationary points $(\Pb^\star, \bom^\star)$, which exist up to re-scaling. This result presents the first landscape analysis of GLA for the joint learning of $(\Pb, \bom)$, while also exploring the stationary points $(\Pb^\star, \bom^\star)$.  In the following, we provide mild conditions on  effective spectral gaps of $\Rb$ and $\bSi$ under which a unique (global) minimum $(\Pb^\star, \bom^\star)$ exists.


\begin{theorem}[Uniqueness of the WPGD Predictor]\label{thm:unique:wpgd} 
Consider independent linear data as given in Definition \ref{def:multitask}. Suppose Assumption~\ref{assum:rb:in:eigenspace} on the correlation vector $\rb$ holds, and 
\begin{align} \label{eqn:gap:cond}
\Delta_{\bSi}\cdot \Delta_{\Rb} <M+s_{\min},    
\end{align}
where \( \Delta_{\bSi} \) and \( \Delta_{\Rb} \) denote the effective spectral gaps of \( \bSi \) and \( \Rb \), respectively, as given in  \eqref{eqn:spec:gap}; \( s_{\min} \) is the smallest eigenvalue of \( \bSi \); and  $M= \sigma^2 + \sum_{i=1}^d s_i$.
\begin{enumerate}[label={\textnormal{\textbf{T\arabic*.}}}, wide, labelindent=0pt, itemsep=0pt]
\item \label{item:fixedpoint} The function \( h_1(h_2(\gamma)) + 1\) is a contraction mapping and admits a unique fixed point \( \gamma = \gamma^\star \).
\item \label{item:globalmin} The loss $\Lc_{\wpgd}(\Pb, \bom)$ has a unique (global) minima $(\Pb^\star, \bom^\star)$, up to re-scaling, given by \eqref{eqn:pstar_and_wstar}.
\end{enumerate}
\end{theorem}
%
\begin{comment}
%% Proof sketch

\textit{Proof sketch}. Let \( \gamma := \frac{\bom^\top \Rb \bom}{\|\bom\|^2}+1 \). Note that \( \gamma \geq 1 \) since \( \Rb \) is positive semi-definite. From the first-order optimality condition, the solution to \eqref{eqn:wpgd:risk} takes the following form:
% \begin{subequations}
\begin{align}\label{eqn:pgamma_and_wgamma}
\Pb(\gamma) &= C(\rb, \bom, \bSi) \cdot \bSi^{-\frac{1}{2}} \left( \frac{\gamma}{M} \cdot \bSi + \Iden \right)^{-1}\bSi^{-\frac{1}{2}}, \quad\text{and}\quad\bom(\gamma) = c(\rb, \bom, \bSi) \cdot \Big(h_2(\gamma) \cdot \Rb + \Iden \Big)^{-1} \rb,    
\end{align}    
% \end{subequations}
for some constants \( C(\rb, \bom, \bSi) \) and \( c(\rb, \bom, \bSi) \).

Substituting the expression for \( \bom(\gamma) \) into \( \gamma = \frac{\bom^\top \Rb \bom}{\|\bom\|^2}+1 \), and applying Assumption~\ref{assum:rb:in:eigenspace}, we obtain the equation \( \gamma = h_1(h_2(\gamma)) +1 \). We then show that whenever \( \Delta_{\bSi} \cdot \Delta_{\Rb} < M + s_{\min} \), the mapping \( h_1(h_2(\gamma)) +1\) is a contraction (see Lemma~\ref{lem:fixedpoint}). By the Banach Fixed-Point Theorem, this guarantees the existence of a unique fixed point \( \gamma = \gamma^\star \), where \( \gamma^\star = h_1(h_2(\gamma^\star)) +1 \). Finally, substituting \( \gamma^\star \) into \eqref{eqn:pgamma_and_wgamma} implies that \( (\Pb^\star, \bom^\star) \), as given in \eqref{eqn:pstar_and_wstar}, is a unique (global) minima of \eqref{eqn:wpgd:risk}, up to re-scaling. See Appendix~\ref{sec:app:wpgd} for the complete proof of Theorem~\ref{thm:unique:wpgd}. \hfill \qed
\end{comment}

Theorem~\ref{thm:unique:wpgd} establishes mild conditions under which a unique (global) minimum $(\Pb^\star, \bom^\star)$ exists, up to scaling invariance, and guarantees the uniqueness of the associated WPGD algorithm. It provides the first global landscape analysis for GLA and generalizes prior work \citep{li2024fine, ahn2024transformers} on the global landscape by extending the optimization properties of linear attention to the more complex GLA with joint $(\Pb, \bom)$ optimization. 

\begin{comment}
\begin{enumerate}[label={\textnormal{\textbf{Remark \arabic*.}}}, wide, labelindent=0pt, itemsep=0pt]
\item \label{item:rem2} 
An interesting observation about the optimal gating parameter $\bom^\star$ is its connection to the correlation matrix $\Rb$, which captures the task correlations in a multitask learning setting. Specifically, the optimal gating given in \eqref{eqn:pstar_and_wstar} highlights how $\bom^\star$ depends directly on both the task correlation matrix $\Rb$ and the vector $\rb$, which encodes the correlations between the tasks and the target task. 
\item \label{item:rem3} Condition~\eqref{eqn:gap:cond} provides a \textit{sufficient} condition for the uniqueness of a fixed point. This implies that whenever $\Delta_{\bSi} \cdot \Delta_{\Rb} < M + s_{\min}$, the mapping $h_1(h_2(\gamma))+1$ is a contraction, ensuring the existence of a unique fixed point. However, there may be cases where the mapping $h_1(h_2(\gamma))+1$ does not satisfy Condition~\eqref{eqn:gap:cond}, yet a unique fixed point (and a unique global minimum) still exists. This is because the Banach Fixed-Point Theorem does not provide a \textit{necessary} condition.
\end{enumerate}
\end{comment}
%




%In the following example, we demonstrate the necessity of Condition~\eqref{eqn:gap:cond} by providing an example that does not satisfy this condition. As a result, the global minima are not unique.

% \begin{example}[]
%  Let \(n = d = 2\). Set \(\lambda_1 = 5\), \(\lambda_2 = 20\), \(a_1 = a_2 = 1\), and \(s_1 = ...  s_2 =... \). In this case, for \(g(\gamma) = 0.5\), the gradient \( \partial h/ \partial g \approx -200\). Additionally, we have \(\Delta_{\Rb} = \lambda_{\max} - \lambda_{\min} = 15\)  and \(\Delta_{\Rb} = \lambda_{\max} - \lambda_{\min} = 15\)  ...
% \end{example}

==> iclr_backup/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
% \def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/fig_iid_k3.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}{0.45\linewidth}    
\centering
\includegraphics[height=0.7\linewidth]{figs/loss.pdf}
\caption{Test risk}\label{fig:loss}
\end{subfigure}
\hspace{20pt}
\begin{subfigure}{0.45\linewidth}    
    \centering
    \includegraphics[height=.7\columnwidth]{figs/corr.pdf}
\caption{Correlation coefficient}\label{fig:corr}
\end{subfigure}
\caption{\textbf{(a)} Train linear attention and GLA models with task-mixture prompts and evaluation results are presented in blue and orange curves, respectively. Here, theory curve (black dotted) is obtained via the Theorem~1 in \cite{li2024fine}. \textbf{(b)} Evolution of correlation coefficients of trained gating parameter $\hat\w_g$ with max-margin solutions obtained in \eqref{w mm}. Here, solid curves represent the results of corr\_coef($\hat\w_g,(\w')^{mm}_g$) where $(\w')^{mm}_g$ is an extended version of $\w^{mm}_g$ following \eqref{w mm extend}. Dashed curves display the results of corr\_coef($\hat\w_g[-d':],\w^{mm}_g$) where $\hat\w_g[-d':]$ returns the last $d'$ dimension of $\hat\w_g$.}\label{fig:iid k3}
\end{figure}


\begin{table}[]
    \centering
    \begin{tabular}{c|ccccc}
    \midrule
        $n$ & $1$ & $5$ & $10$ & $15$ & $20$ \\
    \midrule
        corr\_coef($\hat\w_g,(\w')^{mm}_g$) & $0.962$ & $0.982$ & $0.985$ & $0.988$ & $0.988$\\
    \midrule
        corr\_coef($\hat\w_g[-d':],\w^{mm}_g$) & $0.966$ & $0.996$ & $0.997$ & $0.992$ & $0.994$\\
    \midrule
    \end{tabular}
    \caption{Correlation coefficients of gating parameters with max-margin solutions.}
    \label{tab:iid k3}
\end{table}

==> sec/setup_backup_.tex <==
\section{Problem Setup}

Let $\Z\in\R^{L\times d}$ be the input sequence to a layer, where $L$ is the sequence length and $d$ is the feature dimension. Attention layer embeds $\Z$ into $\Qb,\Kb,\Vb\in\R^{L\times d}$. When we use linear attention with causal mask, the model would output the sequence $\Ob=\text{mask}(\Qb\Kb^\top)\Vb$. Notably, the output of the layer can be computed in a recurrent form as
\begin{align}
&\Sb_{i}=\Sb_{i-1}+\vb_i\kb_i^\top\\
&\ob_i=\Sb_{i}\qb_i.
\end{align}
This recurrent form provides a novel perspective on why linear attention is more efficient than softmax attention and has motivated the design of Gated Linear Attention (GLA)~strategies. 

\noindent\textbf{Gated Linear Attention.} In essence, GLA follows the same structure as linear attention but with a gating mechanism. Let $\Gb_i=g(\z_i)\in\R^{d\times d}$ to be the gating function at time $i$. The GLA can be written in recurrent form as
\begin{align}
&\Sb_{i}=\Gb_i\odot \Sb_{i-1}+\vb_i\kb_i^\top\\
&\ob_i=\Sb_{i}\qb_i.\label{eq:GLA}
\end{align}
Above $\odot$ represents the Hadamard product which does entrywise multiplication. As discussed in the GLA paper [\url{https://arxiv.org/pdf/2312.06635}], distinct choices of $g(\cdot)$ function corresponds to different popular recurrent architectures such as Mamba, Mamba2, RWKV, etc. Crucially, gating allows for parallel training as dicussed in the Mamba and GLA papers. Here, observe that by setting $\Gb_i=\onebb$ or $\Gb_i=\zerobb$, the model has the option to pass or supress the history.

\noindent\textbf{Background on In-context Learning.} The objective of this work is to develop a formal theoretical understanding of GLA with emphasis on its optimization landscape. The landscape of linear attention is well studied in the in-context learning literature. Specifically, suppose tokens encode input-label pairs i.e.~$\z_i=[\x_i,y_i]$ where $\E[y_i\bgl \x_i]=\bt^\top\x_i$ and $\bt$ is the task vector. Suppose $(\z_i)_{i=1}^L$'s are drawn IID conditioned on $\bt$. Under mild assumptions, it can be shown that \cite{} 1 layer of linear attention learns to implement optimally preconditioned gradient descent. That is, on a new token $\x$, the model predicts $\yh=\hat\bt^\top\x$ where $\hat\bt=\W\X^\top\y$, $(\X,\y)$ are the concatenated input-label matrices, and $\W$ is the preconditioning matrix which help the prediction adapt to the task and input distribution.

\subsection{Connecting GLA to WPGD}\label{sec plain wpgd}
\SO{Before jumping to the delimited-prompt setting of \eqref{mtl prompt}, discuss how GLA can implement 1-step of WPGD with gate-induced weights.}

\noindent\textbf{Starting point: Analyze plain WPGD with multiple tasks.} The parameterization \eqref{bom CoR} is still a special form of the general WPGD where $\bom\in\R^{KL}$ is a free variable. Suppose $(\bt_k)_{k=1}^K$ are gaussian vectors with some correlation structure. What is the optimal weighting scheme $\bom$ that minimize the final query risk $\Lc(\Pb,\bom)=\E_{\Z}\left[(y^{(K)}_L-\li\x^{(K)}_L,\Pb\Xb^\top(\bom \odot\yb)\ri)^2\right]$? This should actually be the first problem we should settle. Here, we don't need any delimiters i.e. prompt has the clean form
\begin{align}
\Z=[\Z_1~\Z_2~\cdots~\Z_K],\label{mtl prompt2}
\end{align}
where we get to weight individual elements however we like using unconstrained $\bom\in\R^{KL}$. The below gated form \eqref{mtl prompt} and the simplified gated form become progressively more constrained versions of this problem (which also requires introducing delimiters/contexts $\db_k$ for motivating gating). Note that, to analyze plain WPGD, we don't need delimeters. So this provides a very clean exposition to the paper in terms of \emph{the optimal weighting of heterogeneous context}.

\noindent\textbf{Quick Analysis of Weighted PGD.} Consider a dataset $\X,\y$ of the following form: $y_i=\x_i^\top\bt_i$. $\bt_i,\x\sim\Nn(0,\Iden)$ are independent. Set $\B=[\bt_1~\dots~\bt_n]$. Let $\x$ be the query and $\bt$ be the associated task so that we wish to predict $y=\x^\top \bt$. Define the covariance matrix and correlation
\[ 
\bSi=\frac{1}{d}\E[\B^\top\B],\quad \rb=\frac{1}{d}\E[\B^\top\bt].
\]
The above normalization ensures the entries of $\bSi,\rb$ are between $[-1,1]$ i.e. they correspond to correlation coefficients. To proceed, we are interested in minimizing the WPGD risk
\[ 
\Lc(\w)=\frac{1}{d}\tn{\bt-\X^\top (\w\odot\y)}^2.
\]
Expanding $\X^\top (\w\odot\y)=\sum_{i=1}^n w_i\x_i\x_i^\top\bt_i$, we find that
\begin{align}
\Lc(\w)&=1-\frac{2}{d}\E[\sum_{i=1}^n w_i\bt^\top\x_i\x_i^\top\bt_i]+\frac{1}{d}\E[\sum_{i,j=1}^n w_iw_j\bt_i^\top\x_i\x_i^\top\x_j\x_j^\top\bt_j]\\
&=1-2\w^\top \rb+\w^\top (\bSi+(d+1)\Iden_d)\w.
\end{align}
Using isotropic and independent nature of $\x_i$'s, this implies $(\bSi+(d+1)\Iden_d)\w_\st= \rb$ and $\w_\st=(\bSi+(d+1)\Iden_d)^{-1}\rb$. In the special case where all tasks are identical, we have $\bSi=\onebb_{n\times n}$ and $\rb=\onebb_{n}$ as a result $\w_\st=\frac{1}{n+d+1}\onebb_n$ which recovers the existing results.

%\SO{Check the derivation to make sure correctness, might be missing a factor $d$}

Building on this, we can analyze the joint landscape of weights $\w\in\R^n$ and preconditioned $\Pb$ in the setting $\x_i\sim\Nn(0,\bSi)$ are IID.

\subsection{Investigating optimization landscape of GLA via multitask prompts} The existing work on ICL makes the strong assumption that the context window uniformly follows the same task $\bt$. Here, we will examine relaxations of this assumption and how gating mechanism plays a critical role in adapting to heterogeneous context window containing different tasks. While we can consider a variety of settings, we will focus on the following scenario for clearer exposition.

Consider $K$ different tasks $(\bt_k)_{k=1}^K$ and for each task draw a length $L$ prompt with IID input-label pairs $(\x^{(k)}_i,y^{(k)}_i)_{i,k\geq 1}$ to obtain sequences $(\Z_k)_{k=1}^K$. These sequences are concatenated to form a single prompt. However, we will assume that there are delimiters that separate the task sequences. Specifically, the final prompt is given by 
\begin{align}
\Z=[\Z_1~\db_1~\Z_2~\db_2~\cdots~\db_{K-1}~\Z_K],\label{mtl prompt}
\end{align}
where $(\db_k)_{k=1}^{K-1}$ are the delimiters that determines start/stop of the tasks. We train a GLA model $f_{\W}$ with attention, gating, and prediction head weigts $\W=[\W_K~\W_Q~\W_V,\w_{gate},\vb]$ as follows 
\begin{align}
\Lc(\W,\vb)=\E_{\Z}\left[\sum_{k=1}^K(y^{(k)}_L-\yh_{kL})^2\right].\label{main obj}
\end{align}
where $\yh_{kL}$ is the $kL$'th model output $f_{\W}(\Z)_{kL}=\vb^\top \ob_{kL}$ following \eqref{eq:GLA}. Above, note that we fit only the last token of each task in line with the prior works \cite{}. However and crucially, the prediction of the task $k$ is influenced by the sequences of all earlier tasks resulting in a complex optimization problem that will shed light on the impact of gating. \SO{Rather than sum of $K$ tasks objective \eqref{main obj}, we might want to consider only fitting the final $K$'th task. This might lead to cleaner analysis+insights initially. In \eqref{main obj}, the optimal weights for individual tasks will likely not be perfectly aligned.}
%Specifically, consider a prompt containing 

\textbf{Gating model and theoretical intuitions.} For simplicity, let us consider a sigmoid gating model which can pass or supress the state via $\Gb_i=g_i\onebb_{d\times d}$ where $g_i=\sigma(\w_{gate}^\top\z_i) \in (0,1)$. Our intuition is as follows:
\begin{itemize}
\item Suppose tasks are entirely uncorrelated, that is, $\bt_i$ does not inform $\bt_{j}$ for $j\neq i$. Then, we expect that when the model encounters $\db_k$, the gating mechanism will suppress the history by setting $g(\db_k)=0$ however when encountered by actual task tokens, the model will pass the history by setting $g(\x_i)=1$ and start accumulating the state to infer the task vector in-context.
\begin{itemize}
    \item Under this model, we expect that, the gating weights will converge to a max-margin separator that separates the task tokens from the delimiters to enforce $g(\db_k)=0$ and $g(\x_i)=1$.
\end{itemize}
\item When tasks are correlated, the model can selectively pass the history. In that case, depending on the correlation level between $\bt_1,\bt_2$, the model will intuitively learn a fixed forgetting level $g(\db_1)=\alpha$ so that features of $\bt_1$ can help estimate $\bt_2$ to an extent.
\end{itemize}

\section{Analysis of GLA: Gating Induces Data-Dependent Sample Weighting}

In this section, we will describe how GLA can be formally analyzed under a somewhat simplified but very concrete setting. In a nutshell, we claim that:
\begin{quote}\emph{Training GLA with ICL objective learns data-dependent Weighted PGD.}
\end{quote}
This is distinct from earlier results such as linear attention learning PGD or H3 learning Weighted PGD (WPGD). The crux of GLA is the data-dependence of the weighting procedure. Before describing the details, let us first describe data-dependent WPGD.

\noindent\textbf{Data-dependent WPGD.} Let $(\x_i,y_i)_{i=1}^N$ be a dataset, $\X=[\x_1~\dots~\x_N]^\top$ and $\y=[y_1~\dots~\y_N]$. Also let $\Pb\in\R^{d\times d}$ be the preconditioning matrix and $\bom\in\R^N$ be the weighting vector. The WPGD predictor is given by
\begin{align}
\bt(\Pb,\bom)=\Pb\X^\top (\bom\odot\y).\label{wpgd}
\end{align}
In case of GLA, $\bom$ will be given as a multiplication of data-dependent weights. Specifically, $\bom$ is induced by the gating scalars $g_i:=g(\x_i)$ as follows
\[ 
\omega_i=\prod_{i=1}^{N-1} g(\x_i).
\]
Observe that, crucially, $\x_i$ influences the weighting of all future $\x_{j>i}$. 

\subsection{ICL Analysis of GLA}
We now proceed with describing a concrete technical setting that is amenable to ICL analysis. Our analysis will rely on \emph{decoupling} the influence of gating and data. To this aim, we envision that each token is $\z_t=[y_t,\x_t,\cb_t]$ where $\cb_t\in\R^q$ is the contextual features and $\x_t$ is the predictive features. Additionally,
\begin{itemize}
    \item For task prompts $\Z_i$: Contextual features are set to a fixed vector $\cb_t=\dbb_0\neq 0$.
    %\zerobb_q$. We can easily generalize this to nonzero but fixed contextual features.
    \item For delimeters $\db_i$: Data features are set to zero ($y_i=\x_i=0$) so that $\db_i=[\zerobb_{d+1}~\dbb_i]$ where $\dbb_i$ denotes the context vector.
\end{itemize}
Finally, we assume gating only applies on the context. This ensures that the weighting $\bom$ is independent of the features $\X,\y$ and easier to analyze. Gathering these, we have the following claim. Let
\[ 
\X=[\X_1^\top~\dots~\X_K^\top]^\top,\quad \y=[\y_1^\top~\dots~\y_K^\top]^\top
\]
We claim that attention learns WPGD with weights $\bom$ as in \eqref{wpgd}. Here, the crucial aspect is form of the weighting. $\bom$ takes the following clean form \SO{exponents might be off by 1}.
\[ 
\bom_{kL+i}=g(\dbb_0^\top \w_{gate})^{kL+i-1}\prod_{j=1}^{k-1} g(\dbb_i^\top \w_{gate})
\]
This form follows from the fact that, until $kL+i$, the model observes $kL+i-1$ standard datapoints and $k-1$ delimiters. Now using the shorthand notation $g_0=g(\cb^\top \w_{gate})$ and $g_i=g(\dbb_i^\top \w_{gate})$, we can rewrite
\begin{align}
\bom_{kL+i}=g_0^{kL+i-1} \prod_{j=1}^{k-1}g_i.\label{bom orig}
\end{align}
Whenever $(\dbb_i)_{i=0}^{L-1}$ are linearly independent and gating function is sufficiently expressive\footnote{In case of sigmoid, it can express everything in the [0,1] interval but not the whole real line.}, gating function can be treated as \textbf{unconstrained variables}, that is, model can express any scalars $\g=(g_i)_{i=0}^{K-1}$ of its choice. As a result, the analysis of GLA directly relates to the \emph{risk of optimally-weighted PGD}. 

\noindent\textbf{Change of variable trick.} To further simplify \eqref{bom orig} let us apply a change of variable relying $g'_k\gets g_0^L g_k$ and $\tilde{g}_k=\prod_{j=1}^{k-1}g'_j$. Through this, we obtain the simplified form
\begin{align}
\bom_{kL+i}=g_0^{i-1} \prod_{j=1}^{k-1}g'_j=g_0^{i-1} \tilde{g}_k.\label{bom CoR}
\end{align}
This simplified forms highlight the fact that, along the data sequence $\Z_i$, gating results in an exponential filter whereas and delimeters act as a multiplicative adjustments that can be summarized as $g'_k$ or the aggregate multiplier $\tilde{g}_k$. When $\g=(g_k)_{k=1}^K$ are unconstrained variables, \eqref{bom CoR} is precisely equivalent to the original form \eqref{bom orig}.
 

Suppose $(\X_i,\y_i)_{i=1}^{K}$ are all datasets with IID samples and consider the objective 
\begin{align}\tag{GatingLoss}
\Lc(\Pb,\g)=\sum_{k=1}^K \Lc_k(\Pb,\g):=\sum_{k=1}^K\E[(y^{(k)}_L-\li\x^{(k)}_L,\Pb\Xb_k(\bom^{(k)}\odot\yb_k)\ri)^2.\label{GWPGD}
\end{align}
Above $\Lc_k$ is the $k$'th loss induced by the $i$'th sequences prediction, $\Xb_k,\yb_k$ are the concatenations of $(\X_j,y_j)_{j=1}^k$ (but not including the token $\z^{(k)}_L$) and $\bom^{(k)}$ is the first $Lk-1$ entries of the weight vector $\bom$.

With the formulation of \eqref{GWPGD}, the problem (essentially) boils down to the landscape analysis of the population risk of WPGD to obtain the optimal gating weights $\g=(g_i)_{i=0}^{K-1}$. A major starting/exposition point for the analysis is directly studying the simplified change-of-variable form \eqref{bom CoR} under the unconstrained variable assumption. This brings us to the following claim when the task vectors $(\bt_k)_{k=1}^K$ are independent.

\begin{claim} The optimal choice of $\g$ is given by $g_0=1$ and $g_{k\geq 1}=0$.
\end{claim}
Note that, if this claim holds for the unconstrained variable setting, it automatically holds for the sigmoid gating because optimal function for unconstrained is also optimal for the [0,1] constrained sigmoidal.

Once this is proven, I believe we can then deduce the GLA-WPGD equivance by utilizing the facts that (i) $g_i$'s are independent of features (in fact, even deterministic) and (ii) odd moment statistics that appear in linear attention will vanish. Note that, if task vectors are dependent, then most likely the following claim holds.

\begin{claim}\label{claim2} The optimal choice of $\g$ is given by $g_0=1$ and $g_{k\geq 1}=\alpha_k$ for a suitable choice.
\end{claim}
I recommend proving the above claim first in the setting of $K=2$.

Finally, as a variation of \eqref{GWPGD}, rather than adding $K$ loss terms, we can directly focus on analyzing the $K$'th loss. That is, rather than \eqref{GWPGD}, we study
\begin{align}\tag{SingleLoss}
\Lc(\Pb,\g)=\E[(y^{(K)}_L-\li\x^{(K)}_L,\Pb\Xb_K(\bom^{(K)}\odot\yb_K)\ri)^2.\label{SWPGD}
\end{align}




\subsection{Relaxing Assumptions on Gating (requires fleshing out)}

Above we have been using the assumption that gating only depends on $\cb_t$ and not on $\x_t$. This might appear too simplistic because it kind of circumvents the data-dependent nature of gating by using context $\cb_t$ rather than features $\x_t$. I believe this can be avoided. The basic idea is the following claim:
\begin{claim} Suppose $\y=\X\bt_\star$ and $\omega_t=g(\w_{wgt}^\top\x_t)$. Suppose $\x,\bt\sim\Nn(0,\Iden_d)$. Consider the estimator $\hat\bt=\Pb\X^\top(\bom\odot\y)$. Choosing $g(\cdot)=\texttt{constant}$ is a near-optimal weighting strategy to minimize risk. That is, you want to weight all samples equally and data-dependent weighting don't buy anything (except perhaps $\order{1/d}$ improvements).
\end{claim}
\noindent\textbf{Proof idea.} The proof should follow from rotational invariance of gaussian. Specifically, gating can only contribute to the estimation of $\bt$ along the subspace $\w_{wgt}$. Over the remaining $d-1$ dimensional subspace, unless all weights are equal, gating will only reduce the performance because $\omega_t$ is independent of $\x^\perp_t$, which is the projection of $\x_t$ on the orthogonal complement of $\w_{wgt}$. Note that analysis of gating is more tricky because $\omega_t$ is multiplication of all earlier $g(\w_{gate}^\top\x_{\tau<t})$ rather than a direct function of $\x_t$. \SO{In fact, the actual gated prediction seems nonlinear in the query $\x$. Based on \eqref{eq:GLA}, the prediction seems to include gating of $\x$, namely, $\hat y=g(\x)\x^\top \hat\bt$. This has to be written very accurately.}

\noindent\textbf{Suggestion.} Even if we don't want to worry about proving/formalizing this aspect, we can run experiments to verify the claim. We simply need to run experiment where gating is allowed to be function of $\x_t$ and demonstrate that result doesn't change.

%$\x_t\perp \cb_t$ to keep things clean. I think this assumption is not needed. We only need $\x_t$ of data to be separable from $\db_i$'s

%Finally, imagine the contexts of the individual data points are also arbitrary and resulting gate-weightings are unconstrained. In that case, we can view $\bom$ as a fully unconstrained vector in $\R^{KL}$ and gating becomes precisely equal to weighted.
%and formalize Claim \ref{claim2} for $K=2$.
%\noindent\textbf{Critical assumption 1:} Gating is only a function of $\cb_i$ whereas attention weights only apply on $[\x_i,y_i]$. This can be guaranteed by assuming $\x_i,\cb_i$ lie on orthogonal subspaces. That is, tokens effectively have the form $\z_i=[y_i,\x_i,\cb_i]$.


%\begin{itemize}
%\end{itemize}


